Properties of Inconsistency Measures for Databases

How should we quantify the inconsistency of a database that violates integrity constraints? Proper measures are important for various tasks, such as progress indication and action prioritization in cleaning systems, and reliability estimation for new datasets. To choose an appropriate inconsistency measure, it is important to identify the desired properties in the application and understand which of these is guaranteed or at least expected in practice. For example, in some use cases the inconsistency should reduce if constraints are eliminated; in others it should be stable and avoid jitters and jumps in reaction to small changes in the database. We embark on a systematic investigation of properties for database inconsistency measures. We investigate a collection of basic measures that have been proposed in the past in both the Knowledge Representation and Database communities, analyze their theoretical properties, and empirically observe their behaviour in an experimental study. We also demonstrate how the framework can lead to new inconsistency measures by introducing a new measure that, in contrast to the rest, satisfies all of the properties we consider and can be computed in polynomial time.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> complexity.tex <==
\section{Computational Complexity}\label{sec:complexity}
We now discuss aspects of computational complexity, and begin with the
complexity of measuring inconsistency according to the aforementioned
example measures.
%(the top four rows of
%Table~\ref{table:postulates}). 
We focus on the class of DCs and the
special case of FDs. Moreover, we focus on \e{data complexity}, which
means that the set $\Sigma$ of constraints is fixed, and only the
database $D$ is given as input for the computation of $\I(\Sigma,D)$.

\revone{\textbf{Complexity for $\Id, \Imi, \Ip$.}~} The measure $\Id$ boils down to testing consistency, which is doable
in polynomial time (under data complexity). The measures $\Imi$ and $\Ip$ can be
computed by enumerating all the subsets of $D$ of a bounded size,
where this size is determined by $\Sigma$. Hence, $\Imi$ and $\Ip$ can also be
computed in polynomial time. 
%Yet, the measures $\Imc$, $\Imc'$ and $\Imr$ can be intractable to compute, already in the case of FDs, as we explain next.

\revone{\textbf{Complexity for $\Imc, \Imc'$.}~} \mrev{The measures $\Imc$ and $\Imc'$ %and $\Imr$ 
can be intractable to compute, already in the case of FDs}. When $\Sigma$ is a set of FDs, $\Imc(\Sigma,D)$ is the number of
maximal independent sets (minus one) of the \e{conflict graph} wherein
the tuples of $D$ are the nodes, and there is an edge between every
two tuples that violate an FD. Counting maximal independent sets is
generally \#P-complete, with several tractable classes of graphs such
as the \e{$P_4$-free} graphs that do not have any
induced subgraph that is a path of length
four. %We have proved that, 
Under conventional
complexity assumptions, the finite sets $\Sigma$ of FDs for which
$\Imc(\Sigma,D)$ is computable in polynomial time are \e{precisely}
the sets $\Sigma$ of FDs that entail a $P_4$-free conflict graph for
every database $D$~\cite{DBLP:conf/pods/LivshitsK17}. Note that $\Imc'$ is equivalent to $\Imc$ in the case of FDs; hence, the same applies to $\Imc'$.

\revone{\textbf{Complexity for $\Imr$.}~} \mrev{The measures $\Imr$ 
is also intractable to compute even for FDs}. For $\C=\Cfd$ and $\R=\R_\subseteq$, the measure $\Imr(\Sigma,D)$ is
the size of the minimum \e{vertex cover} of the conflict graph. Again,
this is a hard (NP-hard) computational problem on general graphs. 
In a recent work, it has been shown that there is an efficient procedure that takes as input a set $\Sigma$ of FDs and
determines one of two outcomes: \e{(a)} $\Imr(\Sigma,D)$ can be
computed in polynomial time, \e{or
  (b)} $\Imr(\Sigma,D)$ is NP-hard to compute (and even approximate
beyond some
constant)~\cite{DBLP:conf/pods/LivshitsKR18}. 
%In
%an earlier work~\cite{DBLP:conf/pods/LivshitsKR18}, we have presented
%an efficient procedure that takes as input a set $\Sigma$ of FDs and
%determines one of two outcomes: \e{(a)} $\Imr(\Sigma,D)$ can be
%computed in polynomial time, \e{or
%  (b)} $\Imr(\Sigma,D)$ is NP-hard to compute (and even approximate
%beyond some
%constant). 
%Interestingly, this
%problem turns out to be the same as that of computing the \e{most
%  probable database} of a tuple-independent probabilistic database
%under FD conditions~\cite{GVSBUDA14}, and our work has resolved their
%open problem of completing a dichotomy in
%complexity~\cite{DBLP:conf/pods/LivshitsKR18}. 
There, they have also
studied the case where the repair system allows only to update cells
(and not delete or insert tuples). In both repair systems it is the
case that, if $\Sigma$ consists of a single FD per relation (which is
a commonly studied case, e.g., key
constraints~\cite{DBLP:journals/jcss/FuxmanM07,DBLP:journals/tods/KoutrisW17})
then $\Imr(\Sigma,D)$ can be computed in polynomial time.
Unfortunately, this is no longer true (under conventional complexity
assumptions) if we go beyond FDs to simple EGDs.

\begin{example}\label{example:egds}
Consider the following four EGDs.
{\small
\begin{align*}
  \sigma_1:\quad & \forall {x,y,z}[R(x,y), R(x,z) \Rightarrow (y=z)] \\
  \sigma_2:\quad & \forall {x,y,z}[R(x,y), R(y,z) \Rightarrow
  (x=z)] \\
  \sigma_3:\quad & \forall {x,y,z}[R(x,y), R(y,z) \Rightarrow
  (x=y)] \\
    \sigma_4: \quad & \forall {x,y,z}[R(x,y), S(y,z) \Rightarrow (x=z)] 
\end{align*}
}
Observe that $\sigma_1$ is an FD whereas $\sigma_2$, $\sigma_3$ and
$\sigma_4$ are not. The constraint $\sigma_2$ states that there are no
paths of length two except for two-node cycles, and $\sigma_3$ states
that there are no paths of length two except for single-node
cycles. Computing $\Imr(\Sigma,D)$ w.r.t.~$\Sigma=\set{\sigma_1}$ or
$\Sigma=\set{\sigma_4}$ can be done in polynomial time; however, the
problem becomes NP-hard for $\Sigma=\set{\sigma_2}$ and
$\Sigma=\set{\sigma_3}$.\qed
\end{example}

The next theorem fully classifies the complexity of computing $\Imr(\Sigma,D)$ for $\Sigma$ that consists of a single EGD with two binary atoms.

\def\thmegd{
Let $\R=\R_{\subseteq}$, and let $\Sigma$ be a set that consists of a
single EGD $\sigma$ with two binary atoms. If $\sigma$ is of the
following form:
\begin{align*}
  \forall x_1,x_2,x_3 [R(x_1,x_2), R(x_2,x_3) \Rightarrow (x_i=x_j)]
\end{align*}
then computing $\Imr(\Sigma,D)$ is NP-hard. In any other case, $\Imr(\Sigma,D)$ can be computed in
polynomial time.
}

\begin{theorem}\label{THM:EGD}
 \thmegd
\end{theorem}

The proof of the theorem is given in the extended version~\cite{extended}. We prove the hardness side by reduction from MaxCut---the problem of finding a cut in a graph (i.e., a partition of the vertices into two disjoint subsets), such that the number of edges crossing the cut is the highest among all possible cuts~\cite{10.5555/574848}. We also provide efficient algorithms for the tractable cases. Note that the EGDs $\sigma_2$ and $\sigma_3$ from
Example~\ref{example:egds} satisfy the condition of
Theorem~\ref{THM:EGD}; hence, computing $\Imr(\Sigma,D)$ w.r.t.~these
EGDs is indeed NP-hard. The EGDs $\sigma_1$ and $\sigma_4$ do not satisfy the condition of the theorem; thus,
computing $\Imr(\Sigma,D)$ w.r.t.~these EGDs can be done in polynomial
time.
%\begin{proofsketch}
%We prove the hardness side by reduction from MaxCut---the problem of finding a cut in a graph (i.e., a partition of the vertices into two disjoint subsets), such that the number of edges crossing the cut is the highest among all possible cuts~\cite{10.5555/574848}. Given a graph $g$, we construct a database $D$ by adding two facts $R(\val{1},v)$ and $R(v,\val{2})$ for every vertex $v$ of $g$, and two facts $R(v,u)$ and $R(u,v)$ for every edge $(v,u)$ of $g$. Note that the facts $R(\val{1},v), R(v,\val{2})$ jointly violate every EGD of the given form, and the same holds for $\set{R(\val{1},v),R(v,u)}$, $\set{R(v,\val{2}),R(u,v)}$, and $\set{R(v,u),R(u,w)}$. We set the cost of deleting facts of the form $R(u,v)$ to one, and the cost of deleting $R(\val{1},v)$ or $R(v,\val{2})$ to be high enough, so that it is always less costly to keep (precisely) one of these facts, for every vertex $v$, in a consistent subset of the database. Then, the only other facts that we can keep to preserve consistency correspond to edges $(v,u)$ crossing the edge (one fact for each such edge), and we can compute the number of edges crossing the cut from $\Imr(\Sigma,D)$.

%For the positive side of the theorem, we present polynomial-time algorithms for each one of the remaining cases. A simple example is the case of EGDs of the form:
%$$\forall x_1,x_2,x_3 \big[R(x_1,x_2),
%R(x_1,x_3)\Rightarrow 
%(x_i=x_j)\big]$$
%where we observe that if $x_i=x_2$ and $x_j=x_3$, then this EGD is, in fact, an FD; hence, $\Imr(\Sigma,D)$ can be computed in polynomial time~\cite{DBLP:conf/pods/LivshitsKR18}. If $x_i,x_j\in\set{x_1,x_2}$ or $x_i,x_j\in\set{x_1,x_3}$, then only facts of the form $R(\val{a},\val{a})$ are allowed, and we simply have to remove the rest of the facts from the database.
%\end{proofsketch}

%The full proof of Theorem~\ref{THM:EGD}, as well as efficient algorithms for the tractable cases, are given in the full version of the paper~\cite{extended}. 


==> intro-old.tex <==
\section{Introduction}
Inconsistency of databases may arise in a variety of situations, for a
variety of reasons. Database records may be collected from imprecise
sources (social encyclopedias/networks, sensors attached to
appliances, cameras, etc.)  via imprecise procedures (natural-language
processing, signal processing, image analysis, etc.), or be integrated
from different sources with conflicting information or formats. Common
principled approaches to handling inconsistency consider databases
that violate \e{integrity constraints}, but can nevertheless be
\e{repaired} by means of \e{operations} that revise the database and
resolve inconsistency~\cite{DBLP:conf/pods/ArenasBC99}. Instantiations
of these approaches differ in the supported types of integrity
constraints and operations. The constraints may be Functional
Dependencies (FDs) or the more general Equality-Generating
Dependencies (EGDs)
%~\cite{DBLP:journals/siamcomp/BeeriV84} 
or, even
more generally, Denial Constraints
(DCs)
%~\cite{DBLP:journals/jiis/GaasterlandGM92}, 
and they may be
referential (foreign-key) constraints or the more general inclusion
dependencies~\cite{DBLP:conf/icdt/AfratiK09}.  A repair operation can be a \e{deletion} of a tuple, an
\e{insertion} of a tuple, or an \e{update} of an attribute value.
Operations may be associated with different \e{costs}, representing
levels of trust in data items or extent of
impact~\cite{DBLP:conf/icdt/LopatenkoB07}.

Various approaches and systems have been proposed for data cleaning
and, in particular, data repairing
(e.g.,~\cite{DBLP:journals/pvldb/EbaidEIOQ0Y13,DBLP:journals/pvldb/GeertsMPS13,DBLP:journals/pvldb/RekatsinasCIR17}
to name a few). We explore the question of \e{how to
  measure database inconsistency} in a manner that reflects the
progress of repairing. Inconsistency measures are useful not just for
implementing progress bars in data repair systems, but also for
recommending next steps in interactive systems, and estimating
the potential usefulness and cost of incorporating databases for downstream analytics~\cite{DBLP:conf/edbt/PapottiNK15}.
In a more general perspective, the importance of incorporating progress indicators in interactive systems has been well recognized and studied in the Human-Computer Interaction (HCI) community~\cite{Myers:1985:IPP:317456.317459, Conn:1995:TAT:223904.223928,Harrison:2007:RPB:1294211.1294231,Harrison:2010:FPB:1753326.1753556,Villar:2013:AIM:2542634.2542637}.

Example measures include the number of violations in the database, the
number of tuples involved in violations, and the number of operations
needed to reach consistency. However, for a measure to effectively
communicate \e{progress indication} in repairing, it should feature certain characteristics. For example,
it should minimize jitters, jumps and sudden changes to have a good
correlation with ``the expected waiting time''---an important aspect
in interacting with the users. It should also be computationally
tractable so as not to compromise the efficiency of the repair and to
allow for interactive systems. Luo et al.~\cite{DBLP:conf/sigmod/LuoNEW04}
enunciate the importance of these properties,
referring to them as ``acceptable pacing'' and
``minimal overhead," respectively, 
in progress indicators for database queries.

As a guiding principle, we adopt the approach of \e{rationality
  postulates} of \e{inconsistency measures} over knowledge bases that have been investigated in depth by the Knowledge
Representation (KR) and Logic
communities~\cite{DBLP:conf/ijcai/KoniecznyLM03,DBLP:journals/jolli/Knight03,DBLP:journals/jiis/GrantH06,DBLP:conf/kr/HunterK08,DBLP:journals/ai/HunterK10,DBLP:journals/ijar/GrantH17,DBLP:journals/ki/Thimm17}.
Yet, the studied measures and postulates fall short of capturing our
desiderata, for various reasons. First, inconsistency is typically
measured over a knowledge base of logical sentences (formulas without
free variables).  In databases, we reason about \e{tuples} (facts) and
fixed integrity constraints, and inconsistency typically refers to the
tuples rather than the constraints (which are treated as exogenous
information). In particular, while a collection of sentences might
form a contradiction, a set of tuples can be inconsistent only in the
presence of integrity constraints.  Hence, as recently
acknowledged~\cite{DBLP:journals/corr/abs-1804-08834,DBLP:journals/corr/abs-1904-03403}, it is of
importance to seek inconsistency measures that are closer to database
applications. Perhaps more fundamentally, in order to capture the
repairing \e{process} and corresponding changes to the database, the
measure should be aware of the underlying \e{repairing operations}
(e.g., tuple insertion, deletion, revision).

For illustration, let us consider the case where all constraints are
anti-monotonic (i.e., consistency cannot be violated by deleting
tuples), and we allow only tuple deletions as repairing operations.
One simple measure is the \e{drastic measure} $\Id$, which is $1$ if
the database is inconsistent, and $0$
otherwise~\cite{DBLP:journals/ki/Thimm17}. Of course, this measure
hardly communicates progress, as it does not change until the very
end.  What about the measure $\Ip$ that counts the number of
\e{problematic tuples}, which are the tuples that participate in
(minimal) witnesses of
inconsistency~\cite{DBLP:conf/kr/HunterK08,DBLP:journals/ai/HunterK10}?
This measure suffers from a disproportional reaction to
repairing operations, since the removal of a single tuple (e.g., a
misspelling of a country name) can cause a drastic reduction in
inconsistency.  As another example, take the measure $\Imc$ that
counts the number of maximal consistent subsets. This measure
suffers from various problems: adding constraints can cause a
\e{reduction} in inconsistency, it may fail to reflect change for
\e{any} deletion of a tuple and, again, it may react disproportionally
to a tuple deletion. Moreover, it is is hard to compute (\#P-complete)
already for simple FDs~\cite{DBLP:conf/pods/LivshitsK17}.

In a recent attention in the community of database theory, measures
have been proposed based on the concept of a \e{minimal repair}---the
minimal number of deletions needed to obtain
consistency~\cite{DBLP:conf/sum/Bertossi18}. We refer to this
measure as $\Imr$. Our exploration shows that $\Imr$ indeed satisfies the rationality
criteria that we define later on, and so,
we provide a formal justification to its semantics. Yet, it is again intractable
(NP-hard) even for simple sets of
FDs~\cite{DBLP:conf/pods/LivshitsKR18}. Interestingly, we are able to
show that a \e{linear relaxation} of this measure, which we refer to
as $\Ilmr$, provides a combination of rationality and tractability.

We make a step towards formalizing the features and 
shortcomings of inconsistency measures such as the aforementioned
ones.  We consider four rationality postulates for database
inconsistency in the context of a \e{repair system} (i.e., a space
of weighted repairing operations): \e{positivity}---the measure is
strictly positive if and only if the database is inconsistent;
\e{monotonicity}---inconsistency cannot be reduced by adding
constraints; \e{progression}---we can always find an operation that
reduces inconsistency; and \e{continuity}---a single operation can
have a limited relative impact on inconsistency. We examine a
collection of measures against these postulates, and show that $\Imr$
stands out. Nevertheless, this measure is intractable. In
particular, we show that computing $\Imr$ is hard already for the case
of a single EGD. Finally, we prove that for tuple deletions, $\Ilmr$
satisfies all four postulates and is computable in polynomial time,
even for the general case of arbitrary sets of denial constraints.

\added{In the context of databases, several notions of
rationality postulates (or axioms) for inconsistency measures have been studied in past research. 
For example, Parisi and Grant~\cite{DBLP:journals/corr/abs-1904-03403}  investigated several database inconsistency measures against rationality postulates adapted from the KR community. However, to the 
best of our knowledge, none of the studied postulates
prevents any form of jumps and jitters of the
inconsistency measure. Some other relevant studies have 
focused on different aspects of inconsistency measures 
for databases. Martinez et al.~\cite{10.1007/978-3-540-75256-1_12} introduced axioms that are inherently based on a numerical interpretation of the database values.}
Grant and
Hunter~\cite{DBLP:conf/ecsqaru/GrantH11}
considered
repairing (or \e{resolution}) operators, and focused on the trade-off between inconsistency reduction
and \e{information loss}: an operation is beneficial if it causes a
high reduction in inconsistency alongside a low loss of
information. 
\eat{Instead, our focus here is on measuring \e{progress} of
repairing, and it is an interesting future direction to understand how
the two relate to each other and/or can be combined.} Another complementary problem is that of associating \e{individual facts} with portions  
of the database inconsistency (e.g., the Shapley value of the fact) and using 
these portions to define preferences among repairs, as studied by Yun et al.~\cite{DBLP:conf/ijcai/YunVCB18}.
\eat{In both studies, the rationality postulates are more general and are not tailored towards progress estimation. As an example, Parisi and Grant~\cite{DBLP:journals/corr/abs-1904-03403} consider the \e{free-formula independence} postulate---if a tuple does not participate in a violation, then removing it from the database should not affect the measure. Contrarily, the removal of a tuple that participates in a violation should decrease the value of the measure, as state by the \e{penalty} postulate. Martinez et al.~\cite{10.1007/978-3-540-75256-1_12} focus on postulates based on the variance of values in the database. In contrast, we focus on different rationality postulates that take the repair system into account (i.e., the aforementioned progression and continuity), and the only postulate considered in all three works is the basic positivity postulate.}


The remainder of the paper is organized as follows. We present
preliminary concepts and terminology in Section~\ref{sec:prelim}. We 
consider inconsistency measures in Section~\ref{sec:measure},
their rationality postulates in Section~\ref{sec:postulates}, 
and complexity aspects in Section~\ref{sec:complexity}. In Section~\ref{sec:rational}, we discuss the developments and challenges in designing rational and tractable measures. Finally, we make concluding remarks and discuss directions for future work in Section~\ref{sec:conclusions}. 
%\textforshortversion{
%Missing proofs are in the (anonymous) 
%extended version of the paper~\cite{extended}.}\footnote{\url{https://figshare.com/s/5dbb066b1fd79358fdbc}}


%Implicitly, previous studies have explored instantiations of
%inconsistency measures in databases without considering general
%appropriateness and
%desiderata~\cite{DBLP:conf/pods/LivshitsKR18,DBLP:conf/icdt/KolahiL09,DBLP:conf/pods/LivshitsK17,GVSBUDA14,DBLP:conf/icdt/KimelfeldLP17,DBLP:conf/icdt/LopatenkoB07,DB%LP:journals/is/BertossiBFL08}.


%drawing connections to \e{answer-set
%  programming}~\cite{DBLP:journals/cacm/BrewkaET11}.

%\section{Research Objectives and Expected Significance}


\eat{
Yet, there are some fundamental differences between their notion of
inconsistency measures and what is needed for quality management in
databases. For one, in databases we reason about tuples (facts)
and fixed integrity constraints, and inconsistency typically refers to
the tuples rather than the constraints. In particular, while a
collection of sentences might form a contradiction, a set of tuples can
be inconsistent only in the presence of integrity constraints.
Moreover, the KR measures do not take into consideration the
underlying repair system and repair operations, which may cast some
inconsistencies easier to fix than others.  Hence, as recently
acknowledged~\cite{DBLP:conf/lpnmr/Bertossi19}, it is of
importance to seek inconsistency measures that are closer to database
applications. In addition, there are computational aspects of
databases (e.g., \e{data complexity}~\cite{DBLP:conf/stoc/Vardi82})
that require a special investigation that is absent from prior art.

Facing the above gaps between the existing inconsistency measures and
rationality postulates on the one hand, and the requirements of
progress estimation in data repairing on the other hand, we make a
first step to propose a framework.

Inconsistency measures serve various purposes in the context of
database quality management. This includes \e{progress
  estimation}---quantify the amount of progress done in data cleaning,
and quantify the target quality; \e{next-step suggestion}---recommend
a cleaning action that maximally reduces inconsistency; and \e{quality
  estimation}---how reliable a database is for drawing conclusions
thereof?  For example, a database can be constructed by a careful
human who may still make mistakes, or be generated by an automated
extraction algorithm that aims for high recall (coverage) at the
expense of low precision (frequent errors).

The goal of the proposed research is to develop fundamental principles
for reasoning about database inconsistency measures and proving their
merit, and to devise actual measures that are practically useful,
efficient to compute, and justified by a clear theoretical ground.  We
plan to conduct our research in three directions. First, following
prior art from KR and Logic~\cite{DBLP:journals/ai/HunterK10,DBLP:journals/ki/Thimm17,DBLP:journals/jolli/Knight03,DBLP:conf/ijcai/KoniecznyLM03,DBLP:journals/jar/Lozinskii94},
we will devise \e{rationality postulates} to serve as a yardstick for
the appropriateness of inconsistency measures.  Second, we will use
the postulates as our lenses for examining past measures, and as our
guide for developing new and better ones. Third, we will explore the
trade-off between the rationality of different inconsistency measures
and their computational complexity. We aim for impact on the practice
and systems for database cleaning, and we aim to establish directions
for database theorists at enriching the principles for managing data
quality~\cite{DBLP:series/synthesis/2011Bertossi,DBLP:journals/dagstuhl-manifestos/AbiteboulABBCD018}.

}

==> introduction_back.tex <==
\section{Introduction}
Inconsistency of databases may arise in a variety of situations for a
variety of reasons. Database records may be collected from imprecise
sources (social encyclopedias/networks, sensors attached to
appliances, cameras, etc.)  via imprecise procedures (natural-language
processing, signal processing, image analysis, etc.), or be integrated
from different sources with conflicting information or formats.
Common
principled approaches to handling inconsistency consider databases
that violate \e{integrity constraints}, but can nevertheless be
\e{repaired} by means of \e{operations} that revise the database and
resolve inconsistency~\cite{DBLP:conf/pods/ArenasBC99}.
Instantiations differ in the supported types of integrity constraints, 
allowed operations, and optimization goals. The constraints may be Functional Dependencies (FDs)
or the more general Equality-Generating Dependencies (EGDs)
%~\cite{DBLP:journals/siamcomp/BeeriV84} 
or, more generally, Denial Constraints (DCs)
%~\cite{DBLP:journals/jiis/GaasterlandGM92}, 
and they may be
referential (foreign-key) constraints or the more general inclusion
dependencies~\cite{DBLP:conf/icdt/AfratiK09}.
 A repair operation can be a \e{deletion} of a tuple,
an \e{insertion} of a tuple, or an \e{update} of an attribute value.
Operations may be associated with different \e{costs}, representing
levels of trust in data items or extent of
impact~\cite{DBLP:conf/icdt/LopatenkoB07}. Optimization goals can be minimization of the costs incurred \cite{DBLP:conf/icdt/KolahiL09, DBLP:conf/pods/LivshitsKR18} or producing the most probabable clean database from a distribution \cite{DBLP:journals/pvldb/RekatsinasCIR17} that fully (hard constraints) or partially (soft constraints) fix the violated integrity constraints. 
Various approaches and systems have been proposed for data cleaning
and, in particular, data repairing
(e.g.,~\cite{DBLP:journals/pvldb/EbaidEIOQ0Y13,DBLP:journals/pvldb/GeertsMPS13,DBLP:journals/pvldb/RekatsinasCIR17}
to name a few).


We explore the question of \e{how to measure database inconsistency}.
This question may arise in different situations.  A measure of
inconsistency can be used for estimating the potential usefulness and
cost of incorporating databases for downstream
analytics~\cite{DBLP:conf/edbt/PapottiNK15}.  We can also use an
inconsistency measure for implementing a progress bar for data
repairing.  Indeed, the importance of incorporating progress
indicators in interactive systems has been well recognized and studied
in the Human-Computer Interaction (HCI)
community~\cite{Myers:1985:IPP:317456.317459,
  Conn:1995:TAT:223904.223928,Harrison:2007:RPB:1294211.1294231,Harrison:2010:FPB:1753326.1753556,Villar:2013:AIM:2542634.2542637}.
Beyond the indication of progress, a measure of inconsistency can be
used for prioritizing and recommending actions in data
repairing---address the tuples that have the highest
\e{responsibility} to the inconsistency level (e.g., Shapley value for
inconsistency~\cite{DBLP:journals/ai/HunterK10,DBLP:conf/ijcai/YunVCB18,DBLP:journals/corr/abs-2009-13819})
or the ones that might result in the greatest reduction in
inconsistency.

Example measures include the number of violations in the database, the
number of tuples involved in violations, and the number of operations
needed to reach consistency.  To choose an appropriate inconsistency
measure for a specific use case, it is important to identify the
desired properties of the application and understand which of these is
guaranteed or expected in practice.  For example, to effectively
communicate progress indication in repairing, the measure should
feature certain characteristics. While it should react to changes made in the database and show progress when the database is ``cleaner'' with respect to the given integrity constraints, it should minimize jitters, jumps and
sudden changes in reaction to small changes in the database, and in turn,
should have a good correlation with ``the expected waiting time''---an
important aspect in interacting with the users. 
It should also be
computationally tractable 
%so as not to compromise the efficiency of the repair and 
to allow for interactive systems. Luo et
al.~\cite{DBLP:conf/sigmod/LuoNEW04} enunciate the importance of these
properties, referring to them as ``acceptable pacing'' and ``minimal
overhead," respectively, in progress indicators for database queries.



%We also report on an empirical study of these measures.
%in a manner that reflects the desiderata of different use cases.
%Inconsistency measures are useful not just for implementing
%progress bars in data repair systems,
%but also for recommending next
%steps in interactive systems, 

\begin{figure*}[t]
\subfloat[\small \bf Clean database $D_0$]{
\begin{small}
\begin{tabular}{r|c|c|c|c|c|c|}
\hline
& Id &	Type &	Name &	Continent &	Country &	Municipality	\\
\hline
$f_1$ & 00AA &	Small airport &	Aero B Ranch &		NAm &	US &			Leoti	\\

$f_2$ & 7FA0 &	heliport &	Florida Keys Memorial Hospital Heliport  &	NAm  &	US  &		Key West\\

$f_3$ & 7FA1 &	Small airport &	Sugar Loaf Shores Airport  & NAm  &	US  &	Key West\\

$f_4$ & KEYW &	Medium airport &	Key West International Airport  &	NAm &	US &	Key West\\

$f_5$ & KNQX &	Medium airport &	Naval Air Station Key West/Boca Chica Field  &	NAm &	US  &			Key West\\\hline
\end{tabular}
\end{small}
\label{fig:clean}
}\\
\subfloat[\small \bf Noisy database $D_1$ (bold values are changed from the clean database, underline is used in Figure~\ref{fig:measure-values})]{
\begin{small}
\begin{tabular}{r|c|c|c|c|c|c|}
\hline
& Id &	Type &	Name &	Continent &	Country &	Municipality	\\
\hline
$f_1$ & 00AA &	Small airport &	Aero B Ranch &		NAm &	US &			Leoti	\\

$f_2$ & 7FA0 &	heliport &	Florida Keys Memorial Hospital Heliport  &	{\bf Am}  &	{\bf USA}  &		Key West\\

$f_3$ & 7FA1 &	Small airport &	Sugar Loaf Shores Airport  & \underline{NAm}  &	\underline{US}  &	Key West\\

$f_4$ & KEYW &	Medium airport &	Key West International Airport  &	\underline{NAm} &	{\bf USA} &	Key West\\

$f_5$ & KNQX &	Medium airport &	Naval Air Station Key West/Boca Chica Field  &	{\bf Am} &	\underline{US}  &			Key West\\\hline
\end{tabular}
\end{small}
\label{fig:noisy-1}
}\\
\subfloat[\small \bf Noisy database $D_2$ (bold values are changed from the clean database)]{
\begin{small}
\begin{tabular}{r|c|c|c|c|c|c|}
\hline
& Id &	Type &	Name &	Continent &	Country &	Municipality	\\
\hline
$f_1$ & 00AA &	Small airport &	Aero B Ranch &		NAm &	US &			Leoti	\\

$f_2$ & 7FA0 &	heliport &	Florida Keys Memorial Hospital Heliport  &	{\bf Am}  &	{\bf USA}  &		Key West\\

$f_3$ & 7FA1 &	Small airport &	Sugar Loaf Shores Airport  & NAm  &	US  &	Key West\\

$f_4$ & KEYW &	Medium airport &	Key West International Airport  &	NAm &	{\bf USA} &	Key West\\

$f_5$ & KNQX &	Medium airport &	Naval Air Station Key West/Boca Chica Field  &	NAm &	US  &			Key West\\\hline
\end{tabular}
\end{small}
\label{fig:noisy-2}
}\\
\subfloat[\small \bf Different measure values on two noisy datasets]{
\begin{small}
\begin{tabular}{|c||c|c||c|c||}
\hline
 & \multicolumn{2}{|c||}{Noisy database $D_1$} & \multicolumn{2}{|c||}{Noisy database $D_2$}\\\hline
{\bf Measure} & {\bf value} & {\bf explanation} & {\bf value} & {\bf explanation} \\\hline\hline
$\Id$  &1 & inconsistent database &1 & inconsistent database \\\hline
$\Imr$ (deletions) & 3 & e.g., remove $\{f_2, f_4, f_5\}$ or $\{f_3, f_4, f_5\}$  & 2 & e.g., remove $\{f_2, f_3\}$ or $\{f_2, f_4\}$\\\hline
$\Imr$ (updates) & 4 & change the values shown in {\bf bold} or with an \underline{underline}& 3 & change the values shown in {\bf bold} \\\hline
$\Imi$ & 7 & $|\{\{f_2, f_3\}, \{f_2, f_4\},\{f_2, f_5\}, \{f_3, f_4\},\{f_3, f_5\}, \{f_4, f_5\},\{f_1, f_5\}\}|$   & 5 & $|\{f_2, f_3\}, \{f_2, f_4\},\{f_2, f_5\}, \{f_3, f_4\},\{f_4, f_5\}\}|$ \\\hline
$\Ip$ & 5 & all tuples are involved in violation & 4 & all tuples except $f_1$ are involved in violation \\\hline
$\Imc$ & 3 & $|\{\{f_1, f_2\}, \{f_1, f_3\}, \{f_1, f_4\}, \{f_5\}\}| - 1$ & 2 &  $|\{\{f_1, f_2\}, \{f_1, f_4\}, \{f_1, f_3, f_5\}\}| - 1$  \\\hline
$\Ilmr$ & 2.5 & e.g., assign 0.5 to all $f_1, \cdots, f_5$ (see Section~\ref{sec:lmr}) & 2 & e.g., assign 0.5 to all $f_2, \cdots, f_5$ (see Section~\ref{sec:lmr}) \\\hline
\end{tabular}
\end{small}
\label{fig:measure-values}
}
\caption{\bf A clean and two noisy Airport databases from Example~\ref{eg:running} along with inconsistency measure values.}
%\vspace{-2mm}
\label{fig:running}
\end{figure*}



In this paper, we explore desirable properties of inconsistency measures
and demonstrate the analysis and design of specific inconsistency
measures with respect to these properties.  As a guiding principle, we
adopt the approach of \e{rationality postulates} of \e{inconsistency
  measures} over knowledge bases that have been investigated in depth
by the Knowledge Representation (KR) and Logic
communities~\cite{DBLP:conf/ijcai/KoniecznyLM03,DBLP:journals/jolli/Knight03,DBLP:journals/jiis/GrantH06,DBLP:conf/kr/HunterK08,DBLP:journals/ai/HunterK10,DBLP:journals/ijar/GrantH17,DBLP:journals/ki/Thimm17}.
Yet, the studied measures and postulates fall short of capturing our
desiderata, for various reasons. First, inconsistency is typically
measured over a knowledge base of logical sentences (formulas without
free variables).  In databases, we reason about \e{tuples} (facts) and
fixed integrity constraints, and inconsistency typically refers to the
tuples rather than the constraints (which are treated as exogenous
information). In particular, while a collection of sentences, and even a single sentence, might
form a contradiction, a set of tuples can be inconsistent only in the
presence of integrity constraints.  Hence, as recently
acknowledged~\cite{DBLP:journals/corr/abs-1804-08834,DBLP:journals/corr/abs-1904-03403},
it is of importance to seek inconsistency measures that are closer to
database applications. %Perhaps m
More fundamentally, in order to capture
the repairing \e{process} and corresponding changes to the database,
the measures should be aware of the underlying \e{repairing operations}
(e.g., tuple insertion, deletion, or revision).
\par
The following example illustrates the concept of a noisy database and the differences among certain inconsistency measures that we will discuss in this paper; formal definitions are in Section~\ref{sec:measure}. %\sudeepa{It is a bit late for the example, need to reorganize.}

\begin{example}\label{eg:running}
Consider a simplified version of an 
Airport database\footnote{\url{https://ourairports.com/data/}} over the schema
{\small
$\rel{Airport}(\underline{\att{Id}},\att{Type},\att{Name},\att{Continent},\att{Country},\att{Municipality})$
}
%{\tt Airport(\underline{Id}, Type, Name, 	Continent,	Country,	Municipality)} 
and the following functional dependencies:% (where {\tt muni = municipality}):
{\small
\begin{align*}
    &\att{Municipality}\rightarrow \att{Continent}\,\,\att{Country}\ \ \ \ \ \ \ \
    &\att{Country}\rightarrow \att{Continent}
\end{align*}
}
%
%\sudeepa{is the following format ok?}:
%{\scriptsize
%\begin{itemize}
%\itemsep0em
%    \item ${\mathbf C_1}$:~  {\tt not(t1.id=t2.id)}
%\item ${\mathbf C_2}$:~ ${\tt not(t1.muni=t2.muni \wedge t1.continent!=t2.continent)}$
%\item ${\mathbf C_3}$:~  ${\tt not(t1.muni=t2.muni \wedge t1.country!=t2.country)}$
%\item ${\mathbf C_4}$:~  ${\tt not(t1.continent!=t2.continent \wedge t1.country=t2.country)}$
%\end{itemize}
%}
%The first condition says that $\tt id$ is the key, and the other conditions denote two functional dependencies (FDs)\\ ${\tt muni \rightarrow continent, country}$ and ${\tt country \rightarrow continent}$. 
A clean database $D_0$ where both FDs are satisfied is shown in Figure~\ref{fig:clean}. Figures~\ref{fig:noisy-1} and \ref{fig:noisy-2} show two noisy versions $D_1$ and $D_2$ of the database that violate one or both FDs. It can be seen that $D_1$ has four attribute values changed from $D_0$ (shown in {\bf bold}), whereas $D_2$ has only three values changed. However, an automated data cleaning algorithm cannot directly detect these changes. Using the inconsistency measures discussed in this paper (Section~\ref{sec:measure}), we can see the difference among different measures as shown in Figure~\ref{fig:measure-values}. 
One can notice that some measures do not differentiate these two noisy databases at all, whereas for the others the respective relative values returned are quite different from each other even on this toy database. This in turn raises the question, what the desired properties of an inconsistent measure should be so that we can  compare them with other possible measures, which is the main focus of this paper.  \eat{

We will discuss how the exact values are obtained in Section~\ref{sec:measure}, but looking at the table in Figure~\ref{fig:measure-values}, Among the measures that do differentiate these two noisy databases, $\Imr$ is computationally hard to compute, for both deletions and updates, even for very simple set of integrity constraints \red{CITE}. 
}
\end{example}

\eat{
\red{Ihab: consider moving the below example here and discuss measures $I_i$ against it, for example $I_p$ with the change of x, $I_p$ is decreased by y \%} -- \red{SR: done}
}

\cut{
\red{Ihab: it is hard to see at this stage the disproportional reaction  of $I_p$ as a ``problem''. If we want to say that this makes it hard to use it as a progress indicator, we should spell it out maybe.

Maybe we can say: while $I_p$ tries to reflect more granular measure of inconsistency than $I_d$, there are cases where it can rapidly decrease to 0 with a single repairing action. This lack of ``continuity'' makes it unsuitable to ...}
}

To illustrate some of the inconsistency measures, let us consider the case where all constraints are
anti-monotonic, i.e., consistency cannot be violated by deleting
tuples (e.g., functional dependencies are anti-monotonic whereas referential integrity constraints are not), and we allow only tuple deletions as repairing operations.
One simple measure for such constraints is the \e{drastic measure} $\Id$, which is $1$ if
the database is inconsistent, and $0$
otherwise~\cite{DBLP:journals/ki/Thimm17}. Of course, this measure
hardly communicates progress (both $D_1, D_2$ have $\Id = 1$ as shown in Figure~\ref{fig:measure-values}), as it does not change until the very
end.  %What about the 
Consider another measure $\Ip$ that counts the number of
\e{problematic tuples}, which are the tuples that participate in
\emph{(minimal) witnesses of
inconsistency}~\cite{DBLP:conf/kr/HunterK08,DBLP:journals/ai/HunterK10}, and counting such minimal inconsistent subsets gives yet another measure $\Imi$. 
 Figure~\ref{fig:measure-values} shows both $\Imi$ and $\Ip$ values for $D_1, D_2$; more pairs of tuples are involved in violation of constraints in $D_1$ giving a value of 7 for $\Imi$ on $D_1$, whereas it is 5 for $D_2$. Similarly, all 5 input tuples are ``problematic'' in $D_1$ whereas the number is 4 for $D_2$, leading to the $\Ip$ values. The measure $\Ip$ suffers from a disproportional reaction to repairing
operations: the removal of a single tuple (e.g., a misspelling
of a country name) may cause a drastic reduction in inconsistency. For example, if a single tuple is involved in a conflict with many other tuples, which do not participate in any other violation of the constraints, the removal of this tuple may rapidly reduce the value of this measure from a very high number to
a very low one, and even to zero, as all these tuples are no longer considered ``problematic''.


%, by removing conflicts with many other tuples. If these tuples are not involved in other violations, then this single tuple deletion can rapidly reduce the value of this measure measure to
%zero. %If the tuples are involved in additional violations, the measure


%and making a
%significant progress toward a clean database. However, for $\Ip$, the
%change will be only 1 if the other tuples have other conflicts. On the
%other hand, a single tuple deletion can rapidly reduce this measure to
%zero if there are no other conflicts.

While $\Ip$ attempts to reflect a more granular measure of inconsistency than $\Id$, this disproportionate sensitivity to a single change in the database may or may not work well depending on the application. %\red{SR:plz check Ip}   
As
another example, consider the measure $\Imc$ that counts the number of
\emph{maximal consistent subsets}. Maximal consistent subsets along with the $\Imc$ values for $D_1, D_2$ are shown in Figure~\ref{fig:measure-values}. The measure $\Imc$ suffers from various
problems: adding constraints can cause a \e{reduction} in
inconsistency, it may fail to reflect repairing operations (e.g., it may be the case that the size of a single maximal consistent subset increases in response to a repairing operation, but the number of such subsets remains the same), and, again,
it may react disproportionally to small changes. Moreover, it is 
hard to compute (\#P-complete) already for simple
FDs~\cite{DBLP:conf/pods/LivshitsK17}.  
%While our toy examples in Figure~\ref{fig:measure-values} do not illustrate the 




In a recent attention in the community of database
theory~\cite{DBLP:conf/sum/Bertossi18}, measures have been proposed
based on the concept of a \e{minimal repair}---the minimal number of
 tuple deletions needed to obtain consistency for anti-monotonic constraints. A similar concept is called \emph{update repair}, which repairs a database by updating attribute values rather than deleting tuples as a whole. In general, we denote a measure based on the minimal number of operations required to obtain consistency by $\Imr$. We show that $\Imr$ indeed satisfies the
rationality criteria that we define later on (for both deletions and updates), and so, we provide a
formal justification to its semantics. Yet, it is again intractable
(NP-hard) even for simple sets of
FDs~\cite{DBLP:conf/pods/LivshitsKR18}. Figure~\ref{fig:measure-values} shows the $\Imr$
values for $D_1, D_2$ along with the repairing operations that lead to these values. \\
\cut{
\red{Ihab: Either we make these properties  bold, or separate bullets, I think these definitions are important to be find-able by the reviewer early on.
----
SR -- DONE
----
Also consider moving introduction of $\Ilmr$ from above to after the properties below and mention that not only it is tractable, but also satisfies all 4
----
SR -- DONE
}
}

\noindent
\textbf{Our contributions.~} Given the numerous choices of inconsistency measures for noisy databases one can use, in this paper we ask and address the question what should the desirable properties of an inconsistency measure be, and whether the different notions of inconsistency measures satisfy these properties, so that the user can make an informed choice while adopting one measure vs. another, and can use them in monitoring progress of data repair or recommending a repair operation. We make the following contributions in this paper. 
\cut{
We make a step towards formalizing the behavior of inconsistency
measures such as the aforementioned ones.
}
\par
%{\bf (1) Define and propose meaningful inconsistency measures: } %(better name?) 
%We define inconsistency measures and propose a collection of meaningful inconsistency measures for data repair adopting notions from the KR and Logic literature {(\bf Section~\ref{sec:measure})}.
%\par
{\bf (1) Formalize and analyze desired properties of inconsistency measures: } %and analyze whether different inconsistent measures satisfy these properties: }
We define four properties
for database inconsistency in the context of a \e{repair system} (a space of possibly weighted repairing operations) with the following intuitive meaning:
\begin{enumerate}[label=(\roman*)]
\itemsep0em
    \item {\bf Positivity}: the
measure is strictly positive if and only if the database is
inconsistent,
\item {\bf Monotonicity}: inconsistency cannot be reduced by
adding constraints,
\item {\bf Continuity}: a single operation
can have a limited relative impact on inconsistency, and
\item {\bf Progression}: we can always find an operation
that reduces inconsistency.
\end{enumerate}
Moreover, we use these properties to analyze a  collection of
inconsistency measures known in the KR and Logic literature {(\bf Section~\ref{sec:measure})}.
More specifically, we examine the inconsistency measures against the properties, and show that most of the measures discussed earlier violate one or more of these properties (summarized in Table~\ref{table:postulates}). However, $\Imr$ stands out satisfying all the properties, for both tuple deletions and attribute updates {\bf (Section~\ref{sec:postulates})}. 
\par
{\bf (2) Complexity of measures.} As an additional desideratum for practical purposes, we study the complexity of computing these measures. While many measures are tractable, the measure $\Imr$ that satisfies all the properties is known to be intractable. We show a stronger result that computing $\Imr$ is hard already for the case of a single
EGD  {\bf (Section~\ref{sec:complexity})}. 
\par
{\bf (3) Propose a new measure satisfying all desiderata:}
For tuple deletions, we propose a new measure $\Ilmr$ relaxing the concept of $\Imr$. We show that $\Ilmr$ satisfies all
four properties and is computable in polynomial time, even for the
general case of arbitrary sets of denial constraints, therefore, can provide a combination of rationality and tractability {\bf (Section~\ref{sec:rational})}.

%Interestingly, we are able to show that a \e{linear relaxation} of this measure, which we refer to as $\Ilmr$, provides a combination of rationality and tractability.
\par
{\bf (4) Empirical evaluation of measures:} Our toy example in Figure~\ref{fig:running} is inadequate to show how different measures behave differently with respect to the above desired properties. We empirically evaluate the behavior of these measures on multiple datasets with different integrity constraints and inconsistency levels {\bf (Section~\ref{sec:experiments})}.\\


\noindent
\textbf{Other related work.~} In the context of databases, several notions of rationality
  postulates (or axioms) for inconsistency measures have been studied
  in past research.  For example, Parisi and
  Grant~\cite{DBLP:journals/corr/abs-1904-03403} investigated several
  database inconsistency measures against rationality postulates
  adapted from the KR community. However, to the best of our
  knowledge, none of the studied postulates prevents any form of jumps
  and jitters of the inconsistency measure. Some other relevant
  studies have focused on different aspects of inconsistency measures
  for databases. Martinez et al.~\cite{10.1007/978-3-540-75256-1_12}
  introduced axioms that are inherently based on a numerical
  interpretation of the database values.  Grant and
Hunter~\cite{DBLP:conf/ecsqaru/GrantH11} considered repairing (or
\e{resolution}) operators, and focused on the trade-off between
inconsistency reduction and \e{information loss}: an operation is
beneficial if it causes a high reduction in inconsistency alongside a
low loss of information.  \eat{Instead, our focus here is on measuring
  \e{progress} of repairing, and it is an interesting future direction
  to understand how the two relate to each other and/or can be
  combined.} Another complementary problem is that of associating
\e{individual facts} with portions of the database inconsistency
(e.g., the Shapley value of the fact) and using these portions to
define preferences among repairs, as studied by Yun et
al.~\cite{DBLP:conf/ijcai/YunVCB18}.  \eat{In both studies, the
  rationality postulates are more general and are not tailored towards
  progress estimation. As an example, Parisi and
  Grant~\cite{DBLP:journals/corr/abs-1904-03403} consider the
  \e{free-formula independence} postulate---if a tuple does not
  participate in a violation, then removing it from the database
  should not affect the measure. Contrarily, the removal of a tuple
  that participates in a violation should decrease the value of the
  measure, as state by the \e{penalty} postulate. Martinez et
  al.~\cite{10.1007/978-3-540-75256-1_12} focus on postulates based on
  the variance of values in the database. In contrast, we focus on
  properties that take the repair system into account (i.e., the
  aforementioned progression and continuity), and the only postulate
  considered in all three works is the basic positivity postulate.}


\cut{The remainder of the paper is organized as follows. We present
preliminary concepts and terminology in Section~\ref{sec:prelim}. We
consider inconsistency measures in Section~\ref{sec:measure}, their
properties in Section~\ref{sec:postulates}, and complexity aspects in
Section~\ref{sec:complexity}. In Section~\ref{sec:rational}, we
discuss the developments and challenges in designing tractable
measures. We describe an experimental evaluation in
Section~\ref{sec:experiments}.  Finally, we make concluding remarks
and discuss directions for future work in
Section~\ref{sec:conclusions}.
}

\cut{
\red{serious study of properties of inconsistency measures with empirical evaluation -- the KR community did not look at databases -- repair system needed for sensitivity analysis -- then formal analysis -- and empirical study -- refer to the experiments to see the strange behaviors except running time -- why would you choose one vs. the other?}
}
%\textforshortversion{
%Missing proofs are in the (anonymous) 
%extended version of the paper~\cite{extended}.}\footnote{\url{https://figshare.com/s/5dbb066b1fd79358fdbc}}


%Implicitly, previous studies have explored instantiations of
%inconsistency measures in databases without considering general
%appropriateness and
%desiderata~\cite{DBLP:conf/pods/LivshitsKR18,DBLP:conf/icdt/KolahiL09,DBLP:conf/pods/LivshitsK17,GVSBUDA14,DBLP:conf/icdt/KimelfeldLP17,DBLP:conf/icdt/LopatenkoB07,DB%LP:journals/is/BertossiBFL08}.


%drawing connections to \e{answer-set
%  programming}~\cite{DBLP:journals/cacm/BrewkaET11}.

%\section{Research Objectives and Expected Significance}


\eat{
Yet, there are some fundamental differences between their notion of
inconsistency measures and what is needed for quality management in
databases. For one, in databases we reason about tuples (facts)
and fixed integrity constraints, and inconsistency typically refers to
the tuples rather than the constraints. In particular, while a
collection of sentences might form a contradiction, a set of tuples can
be inconsistent only in the presence of integrity constraints.
Moreover, the KR measures do not take into consideration the
underlying repair system and repair operations, which may cast some
inconsistencies easier to fix than others.  Hence, as recently
acknowledged~\cite{DBLP:conf/lpnmr/Bertossi19}, it is of
importance to seek inconsistency measures that are closer to database
applications. In addition, there are computational aspects of
databases (e.g., \e{data complexity}~\cite{DBLP:conf/stoc/Vardi82})
that require a special investigation that is absent from prior art.

Facing the above gaps between the existing inconsistency measures and
rationality postulates on the one hand, and the requirements of
progress estimation in data repairing on the other hand, we make a
first step to propose a framework.

Inconsistency measures serve various purposes in the context of
database quality management. This includes \e{progress
  estimation}---quantify the amount of progress done in data cleaning,
and quantify the target quality; \e{next-step suggestion}---recommend
a cleaning action that maximally reduces inconsistency; and \e{quality
  estimation}---how reliable a database is for drawing conclusions
thereof?  For example, a database can be constructed by a careful
human who may still make mistakes, or be generated by an automated
extraction algorithm that aims for high recall (coverage) at the
expense of low precision (frequent errors).

The goal of the proposed research is to develop fundamental principles
for reasoning about database inconsistency measures and proving their
merit, and to devise actual measures that are practically useful,
efficient to compute, and justified by a clear theoretical ground.  We
plan to conduct our research in three directions. First, following
prior art from KR and Logic~\cite{DBLP:journals/ai/HunterK10,DBLP:journals/ki/Thimm17,DBLP:journals/jolli/Knight03,DBLP:conf/ijcai/KoniecznyLM03,DBLP:journals/jar/Lozinskii94},
we will devise \e{rationality postulates} to serve as a yardstick for
the appropriateness of inconsistency measures.  Second, we will use
the postulates as our lenses for examining past measures, and as our
guide for developing new and better ones. Third, we will explore the
trade-off between the rationality of different inconsistency measures
and their computational complexity. We aim for impact on the practice
and systems for database cleaning, and we aim to establish directions
for database theorists at enriching the principles for managing data
quality~\cite{DBLP:series/synthesis/2011Bertossi,DBLP:journals/dagstuhl-manifestos/AbiteboulABBCD018}.

}

==> measures_back.tex <==
\section{Inconsistency Measures}\label{sec:measure}
Let $\scs$ be a schema and $\C$ a constraint system. An
\e{inconsistency measure} is a function $\I$ that maps a finite set
$\Sigma\subseteq\C$ of integrity constraints and a database $D$ to a
number $\I(\Sigma,D)\in[0,\infty)$.
Intuitively, a high $\I(\Sigma,D)$ implies that $D$ is far from
satisfying $\Sigma$. We make two standard requirements:
\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item $\I$ is zero on consistent databases; that is, $\I(\Sigma,D)=0$
  whenever $D\models\Sigma$;
\item $\I$ is invariant under logical equivalence of constraints; that
  is, $\I(\Sigma,D) = \I(\Sigma',D)$ whenever $\Sigma\equiv\Sigma'$.
\end{itemize}



%\paragraph*{Examples of Measures}
Next, we discuss several examples of inconsistency measures. Some of these
measures (namely, $\Id$, $\Imi$, $\Ip$ and $\Imc$) are adjusted from the
survey of Thimm~\cite{DBLP:journals/ki/Thimm17}. The simplest
measure is the \e{drastic inconsistency value}, denoted $\Id$, which is the
indicator function of inconsistency.

\[
\Id(\Sigma,D) \eqdef 
\begin{cases}
0 & \mbox{if $D\models\Sigma$;}\\
1 & \mbox{otherwise.}
\end{cases}
\]

%\begin{example}\label{eg:Id}
%In Figure~\ref{fig:running}, $D_0 \models \Sigma$ in Example~\ref{eg:running}, $D_1, D_2$ do not. Hence, $\Id(\Sigma,D_0) = 0$ and $\Id(\Sigma,D_0) = \Id(\Sigma,D_1) = 1$ in Figure~\ref{fig:measure-values}.
%\end{example}

The next measure assumes an underlying repair system $\R$ and constraint system $\C$ such that $\C$ is realizable by
$\R$.  The measure $\Imr$ is the minimal cost of a sequence of
operations that repairs the database. It captures the intuition around
various notions of repairs known as \e{cardinality} repairs and
\e{optimal}
repairs~\cite{DBLP:conf/icdt/KolahiL09,DBLP:conf/pods/LivshitsKR18,DBLP:conf/icdt/AfratiK09}.
\[
\Imr(\Sigma,D) \eqdef \min\set{\kappa\str(o,D)\mid o\in O\str\mbox{ and }
  o(D)\models\Sigma}
\]
This measure is the same as the \e{d-hit} inconsistency measure introduced by Grant and Hunter~\cite{DBLP:conf/ecsqaru/GrantH13}. Moreover, $\Imr$ is the \e{distance from satisfaction} used in property
  testing~\cite{DBLP:journals/jacm/GoldreichGR98}
in the special case where the repair system consists of unit-cost
insertions and deletions.
\par
%When it is clear from the context, we will use $\Imr(\Sigma,D)$ for repairs with deletion, i.e., when the operations $o$ are limited to \emph{tuple deletions} only (called the \emph{optimal subset repair}).
%\cite{DBLP:conf/icdt/KolahiL09, DBLP:conf/pods/LivshitsKR18}. 
%{\small
%\[
%\Imr(\Sigma,D) \eqdef \min\set{\kappa\str(o,D)\mid o\in O\str\mbox{ is a tuple deletion and }
%  o(D)\models\Sigma}
%\]
%}
%If the operations $o$ are limited to \emph{attribute update} only, we get the measure called the \emph{optimal update repair}. 
%{\small
%\[
%\Imrupdate(\Sigma,D) \eqdef \min\set{\kappa\str(o,D)\mid o\in O\str\mbox{ is an attribute update and }
%  o(D)\models\Sigma}
%\]
%}
\begin{example}\label{eg:repair2}
Consider again the databases of Figure~\ref{fig:running} and the set $\Sigma$ of FDs defined in Example~\ref{eg:running}. It holds that $D_0\models\Sigma$, while $D_1\not\models\Sigma$ and $D_2\not\models\Sigma$; hence, $\Id(\Sigma,D_0) = 0$ and $\Id(\Sigma,D_1) = \Id(\Sigma,D_2) = 1$. The values of the measure $\Imr$ on all three databases are given in Figure~\ref{fig:measure-values} for the case where only tuple deletions are allowed as well as the case where the allowed operations are attribute updates. For example, in $D_1$, all pairs of facts from $\set{f_2,f_3,f_4,f_5}$ jointly violate $\Sigma$; thus, only one of these facts may appear in a repair, and the minimal number of facts that we need to remove from the database to satisfy $\Sigma$ is three (e.g., remove $\{f_2,f_4,f_5\}$). Assuming unit-cost deletions, we have that $\Imr(\Sigma,D_1)=3$ for the repair system $\R_\subseteq$. If we consider attribute updates, we need to update at least every bold value in $D_1$ to satisfy the FD $\att{Municipality}\rightarrow \att{Continent}\,\,\att{Country}$; hence, in this case, $\Imr(\Sigma,D_1)=4$ (again, for the case of unit-cost updates).
%Example~\ref{eg:running}, $D_1, D_2$ do not. Hence, $\Id(\Sigma,D_0) = 0$ and $\Id(\Sigma,D_0) = \Id(\Sigma,D_1) = 1$ in Figure~\ref{fig:measure-values}.
%In Figure~\ref{fig:running}, $\Imrsubset(\Sigma,D_0) = \Imrupdate(\Sigma,D_0) = 0$. $\Imrsubset$ and $\Imrupdate$ values for $D_1, D_2$ are shown in Figure~\ref{fig:measure-values} along with the deletions/updates that lead to these values. 
\end{example}

\paragraph*{Measures for anti-monotonic constraints.}
The next measures apply to systems $\C$ of \e{anti-monotonic}
constraints. Recall that an integrity constraint $\sigma$ is
anti-monotonic if for all databases $D$ and $D'$, if
$D\subseteq D'$ and $D'\models\sigma$, then $D\models\sigma$.
Examples of anti-monotonic constraints are the \e{Denial Constraints}
(DCs)~\cite{DBLP:journals/jiis/GaasterlandGM92},
the classic \e{Functional Dependencies} (FDs), \e{conditional
  FDs}~\cite{DBLP:conf/icde/BohannonFGJK07}, and \e{Equality
  Generating Dependencies} (EGDs)~\cite{DBLP:conf/icalp/BeeriV81}.


For a set $\Sigma\subseteq\C$ of constraints and a database
$D$, denote by $\MI_\Sigma(D)$ the set of all \e{minimal
  inconsistent} subsets of $D$; that is, the set of all $E\subseteq D$
such that $E\not\models\Sigma$ and, moreover, $E'\models\Sigma$ for
all $E'\subsetneq E$. Again using our assumption that
constraints are anti-monotonic, it holds that $D\models\Sigma$ if and
only if $\MI_\Sigma(D)$ is empty.  Drawing from known inconsistency
measures~\cite{DBLP:conf/kr/HunterK08,DBLP:journals/ai/HunterK10}, the
measure $\Imi$, also known as \e{MI Shapley Inconsistency},
is the cardinality of this set.
\[\Imi(\Sigma,D) \eqdef |\MI_{\Sigma}(D)|\]
%\sudeepa{Need to say minimum size instead of minimal. Minimal size may not be unique.}
A fact $f$ that belongs to a minimal inconsistent subset $K$
(that is, $f\in K\in\MI_\Sigma(D)$) is called 
\e{problematic}, and the measure $\Ip$ counts the problematic
facts~\cite{DBLP:conf/ecsqaru/GrantH11}.
\[\Ip(\Sigma,D) \eqdef |\cup\MI_\Sigma(D)|\]
%\sudeepa{Again need to clarify minimal or minimum.}

\begin{example}\label{eg:MI_P}
The set $\Sigma$ of constraints of Example~\ref{eg:running} consists of FDs, which are violated by pairs of facts; thus, the size of any minimal inconsistent subset w.r.t.~$\Sigma$ is two.
Since the database $D_0$ of Figure~\ref{fig:running} satisfies $\Sigma$, we have that $\Imi(\Sigma,D_0) = \Ip(\Sigma,D_0) = 0$. As mentioned in Example~\ref{eg:repair2}, in the database $D_1$, all pairs of facts from $\set{f_2,f_3,f_4,f_5}$ jointly violate $\Sigma$, and there are six such pairs. Moreover, $\set{f_1,f_5}$ violates the FD $\att{Country}\rightarrow\att{Continent}$ in $\Sigma$; hence, there are seven violating pairs in total and $\Imi(\Sigma,D_0)=7$. As every fact of $D_1$ occurs in at least one violating pair, we have that $\Ip(\Sigma,D_0)=5$.
%In Figure~\ref{fig:running}, $\Imi(\Sigma,D_0) = \Ip(\Sigma,D_0) = 0$ as $\MI_\Sigma(D_0) = \emptyset$.  $\Imi$ and $\Ip$ values for $D_1, D_2$ are shown in Figure~\ref{fig:measure-values}. As the constraints violated in the noisy databases are FDs, a pair of tuples can violate such FDs, and therefore, the size of any minimal inconsistent subset is 2. The number of such subsets in $\MI_\Sigma(D_1)$ is 7 and in $\MI_\Sigma(D_2)$ is 5. Further, $\cup\MI_\Sigma(D_1) = \{f_1, \cdots, f_5\}$ and $\cup\MI_\Sigma(D_2) = \{f_2, \cdots, f_5\}$, leading to $\Ip$ values of 5 and 4 for $D_1, D_2$ respectively.
\end{example}

For a finite set $\Sigma\subseteq\C$ of constraints and a database
$D$, we denote by $\MC_\Sigma(D)$ the set of all \e{maximal
  consistent} subsets of $D$; that is, the set of all $E\subseteq D$
such that $E\models\Sigma$ and, moreover, $E'\not\models\Sigma$
whenever $E\subsetneq E'\subseteq D$.  Observe that if
$D\models\Sigma$, then $\MC_\Sigma(D)$ is simply the singleton
$\set{D}$. Moreover, under the assumption that constraints are
anti-monotonic, the set $\MC_\Sigma(D)$ is never empty (since, e.g.,
the empty set is consistent). The measure $\Imc$ is the cardinality of
$\MC_\Sigma(D)$, minus one.
\[\Imc(\Sigma,D) \eqdef |\MC_{\Sigma}(D)|-1\]

\added{We note that the definition of $\Imc$ in the KR setting is slightly different than ours, as it takes into account the number of self-contradictions in the knowledge base~\cite{DBLP:conf/ecsqaru/GrantH11,DBLP:journals/ijar/GrantH17}. This highlights an important difference between the standard KR setting and ours. As mentioned before, we distinguish between tuples and integrity constraints, and we measure only tuple sets; hence, no self-contradictions exist per se---an individual tuple is always consistent. However, a tuple can be self-inconsistent in the presence of a relevant constraint (e.g., the DC ``$\mbox{height}>0$''). Parisi and Grant~\cite{DBLP:journals/corr/abs-1904-03403} refer to such tuples as \e{contradictory} tuples. Hence, we also consider here another variant of $\Imc$ that counts \e{self-inconsistencies}, and is defined as follows.
%\sudeepa{Here seems to be maximal and not maximum.}
\[\Imc'(\Sigma,D) \eqdef |\MC_{\Sigma}(D)|+|\SI(D)|-1\]}

\begin{example}\label{eg:MC}
In Figure~\ref{fig:running}, it holds that $\Imc(\Sigma,D_0) = 0$ as $D_0$ is consistent and $\MC_\Sigma(D_0) = \{D_0\}$. The $\Imc$ values for $D_1, D_2$ are shown in Figure~\ref{fig:measure-values} along with the maximal consistent subsets. For instance, for $D_1$, the set $\{f_1, f_2\}$ is a maximal consistent subset as adding $f_3$ introduces a violation of the FD $\att{Municipality}\rightarrow \att{Continent}\,\,\att{Country}$, and the addition of $f_4$ or $f_5$ introduces violations of both FD. As we consider FDs, for which there are no self-inconsistencies, for $D_0, D_1, D_2$, the $\Imc'$ and  $\Imc$ values are the same.
\end{example}




==> preliminaries__Benny_Kimelfeld_s_conflicted_copy_2020-09-22_.tex <==
\section{Preliminaries}\label{sec:prelim}
We first give the basic terminology and concepts.

\subsection*{Relational Model}
A \e{relation signature} is a sequence $\alpha=(A_1,\dots,A_k)$ of
 \e{attributes} $A_i$, where $k$ is the \e{arity} of
$\alpha$. A \e{relational schema} (or just \e{schema} for short)
$\scs$ has a finite set of \e{relation symbols} $R$, each associated with a signature that we denote by $\sig(R)$.
If $\sig(R)$ has arity $k$, then we say that $R$ is $k$-ary.  A
\e{fact} $f$ over $\scs$ is an expression of the form
$R(c_1,\dots,c_k)$, where $R$ is a $k$-ary relation symbol of $\scs$,
and $c_1$,\dots, $c_k$ are \e{values}. When $\scs$ is irrelevant or
clear from the context, we may call a fact over $\scs$ simply a
\e{fact}.  If $f=R(c_1,\dots,c_k)$ is a fact and
$\sig(R)=(A_1,\dots,A_k)$, then we refer to the value $c_i$ as $f.A_i$.

%(where $i=1,\dots,k$).

A \e{database} $D$ over $\scs$ is a mapping from a finite set
$\tids(D)$ of \e{record identifiers} to facts over $\scs$. The set of all databases over a schema
$\scs$ is denoted by $\dbs(\scs)$.  We denote by $D[i]$ the fact that
$D$ maps to the identifier $i$. A database $D$ is a \e{subset} of a
database $E_1$, denoted $D\subseteq E_1$, if
$\tids(D)\subseteq\tids(E_1)$ and $D[i]=E_1[i]$ for all $i\in\tids(D)$.

An \e{integrity constraint} is a first-order sentence over $\scs$. A
database $D$ satisfies a set $\Sigma$ of integrity constraints,
denoted $D\models\Sigma$, if $D$ satisfies every constraint
$\sigma\in\Sigma$. If $\Sigma$ and $\Sigma'$ are sets of integrity
constraints, then we write $\Sigma\models\Sigma'$ to denote that
$\Sigma$ \e{entails} $\Sigma'$; that is, every database that satisfies
$\Sigma$ also satisfies $\Sigma'$. We also write $\Sigma\equiv\Sigma'$
to denote that $\Sigma$ and $\Sigma'$ are \e{equivalent}, that is,
$\Sigma\models\Sigma'$ and $\Sigma'\models\Sigma$. By a \e{constraint
  system} we refer to a class $\C$ of integrity constraints (e.g., the
class of all functional dependencies).

As a special case, a \e{Functional Dependency} (FD) $R:X\rightarrow Y$, where $R$ is a relation symbol and $X,Y\subseteq\sig(R)$, states that every two facts that agree on (i.e., have equal values in) every attribute in $X$ should also agree on every attribute in $Y$. The more general \e{Equality Generating Dependency} (EGD) has the form $$\forall\vec x\left[\varphi_1(\vec x)\wedge\dots\wedge\varphi_k(\vec x)\rightarrow (y_1=y_2)\right]$$ where each $\varphi_j(\vec x)$ is an atomic formula over the schema and $y_1$ and $y_2$ are variables in $\vec x$. Finally, a \e{Denial Constraint} (DC) has the form $$\forall\vec x\neg\left[\varphi_1(\vec x)\wedge\dots\wedge\varphi_k(\vec x)\wedge\psi(\vec x)\right]$$ where each $\varphi_j(\vec x)$ is an atomic formula and $\psi(\vec x)$ is a conjunction of atomic comparisons over $\vec x$.

\begin{example}\label{eg:db-constraints}
%\ester{I am not sure that we need this example}
In Figure~\ref{fig:running}, we have a single 5-ary relation symbol $\rel{Airport}$. All databases have five facts with $\tids(D) = \{f_1, \cdots, f_5\}$. The set of integrity constraints $\Sigma$, which consists of two FDs, is given in Example~\ref{eg:running}.  
\end{example}

\subsection*{Repair Systems}
Let $\scs$ be a schema. A \e{repairing operation} (or just
\e{operation}) $o$ transforms a database $D$ over $\scs$ into another
database $o(D)$ over $\scs$, that is,
$o:\dbs(\scs)\rightarrow\dbs(\scs)$. An example is \e{tuple deletion},
denoted $\del{i}{\cdot}$, parameterized by a tuple identifier $i$ and
applicable to a database $D$ if $i\in\tids(D)$; the result
$\del{i}{D}$ is obtained from $D$ by deleting the tuple identifier $i$
(along with the corresponding fact $D[i]$).  Another example is
\e{tuple insertion}, denoted $\ins{f}{\cdot}$, parameterized by a fact
$f$; the result $\ins{f}{D}$ is obtained from $D$ by adding $f$ with a
new tuple identifier. (For convenience, this is the minimal integer
$i$ such that $i\notin\tids(D)$.) A third example is \e{attribute
  update}, denoted $\upd{i.A}{c}{\cdot}$, parameterized by a tuple
identifier $i$, an attribute $A$, and a value $c$, and applicable to
$D$ if $i\in\tids(D)$ and $A$ is an attribute of the fact $D[i]$; the
result $\upd{i.A}{c}{D}$ is obtained from $D$ by setting the value
$D[i].A$ to $c$. By convention, if $o$ is not applicable to $D$, then
it keeps $D$ intact, that is, $o(D)=D$.

A \e{repair system} (over a schema $\scs$) is a collection of
repairing operations with an associated \e{cost} of applying to a
given database. For example, a smaller change of value might be less
costly than a greater one~\cite{DBLP:conf/lid/GardeziBK11}, and some
facts might be more costly than others to
delete~\cite{DBLP:conf/icdt/LopatenkoB07,DBLP:conf/pods/LivshitsKR18}
or
update~\cite{DBLP:conf/icdt/KolahiL09,DBLP:conf/pods/LivshitsKR18,DBLP:journals/is/BertossiBFL08};
changing a person's zip code might be less costly than changing the
person's country, which, in turn, might be less costly than deleting
the entire person's record.  Formally, a repair system $\R$ is a pair
$(O,\kappa)$ where $O$ is a set of operations and
$\kappa:O\times\dbs(\scs)\ra[0,\infty)$ is a cost function that
assigns the cost $\kappa(o,D)$ to applying $o$ to $D$. We require that
$\kappa(o,D)=0$ if and only if $D=o(D)$; that is, the cost is nonzero
when, and only when, an actual change occurs.

For a repair system $\R$, we denote by $\R\str=(O\str,\kappa\str)$ the repair system 
of all \e{sequences} of operations from $\R$, where the cost
of a sequence is the sum of costs of the individual operations
thereof. 
\textforlongversion{
Formally, for $\R=(O,\kappa)$, the repair system $\R\str$ is
$(O\str,\kappa\str)$, where $O\str$ consists of all compositions
$o=o_m\circ\dots\circ o_1$, with $o_j\in O$ for all $j=1,\dots,m$,
defined inductively by $o_m\circ\dots\circ
o_1(D)=o_m(o_{m-1}\circ\dots\circ o_1(D))$ and
$\kappa\str(o_m\circ\dots\circ
o_1,D)=\kappa(o_m,o_{m-1}\circ\dots\circ
o_1(D))+\kappa\str(o_{m-1}\circ\dots\circ o_1,D)$.
}
Let $\C$ be a constraint system and $\R$ a repair system. We say that
$\C$ is \e{realizable by} $\R$ if it is always possible to make a
database satisfy the constraints of $\C$ by repeatedly applying operations
from $\R$. Formally, $\C$ is realizable by $\R$ if for every database
$D$ and a finite set $\Sigma\subseteq\C$ there is a sequence $o$ in
$\R\str$ such that $o(D)\models\Sigma$.  An example of $\C$ is the
system $\Cfd$ of all FDs $R:X\ra Y$.
%, where $R$ is a relational symbol
%and $X,Y\subseteq\sig(R)$, stating that every two facts that agree on
%(i.e., have equal values in) every attribute in $X$ also agree on
%every attribute in $Y$.  
An example of $\R$ is the \e{subset} system,
denoted $\R_\subseteq$, where $O$ is the set of all tuple deletions
(hence, the result is always a subset of the original database), and
$\kappa$ is determined by a special \e{cost} attribute,
$\kappa(\del{i}{D})=D[i].\mathtt{cost}$, if a cost attribute exists, and otherwise,
$\kappa(\del{i}{D})=1$ (every tuple has unit cost for  deletion). Observe that $\R_\subseteq$ realizes $\C$,
since the latter consists of anti-monotonic constraints.

\begin{example}\label{eg:repair}
The database $D_1$ of Figure~\ref{fig:noisy-1} may be obtained from $D_0$ by applying the following sequence of attribute updates (here, we assume that the identifier of a fact $f_i$ is $i$):
\begin{align*}
    &E_1=\upd{2.\att{Continent}}{\val{Am}}{D_0}\\
    &E_2=\upd{2.\att{Country}}{\val{USA}}{E_1}\\
    &E_3=\upd{4.\att{Country}}{\val{USA}}{E_2}\\
    &D_1=\upd{5.\att{Continent}}{\val{Am}}{E_3}
\end{align*}
If we consider tuple deletions (i.e., the repair system $\R_\subseteq$), we may obtain $D_1$ from $D_0$ by applying the following sequence of operations:
{\small
\begin{align*}
    &E_1=\del{2}{D_0}\,\,\,\,\,\,\,\,\,\,\,\,
    E_2=\ins{f_2}{E_1}\\
    &E_3=\del{4}{E_2}\,\,\,\,\,\,\,\,\,\,\,\,
    E_4=\ins{f_4}{E_3}\\
    &E_5=\del{5}{E_4}\,\,\,\,\,\,\,\,\,\,\,\,
    D_1=\ins{f_5}{E_5}
\end{align*}
}
where $f_2,f_4$ and $f_5$ are the facts of the database $D_1$. We may also assign a cost to each one of these operations. For example, if both tuple deletions and attribute updates are allowed, we may associate a higher cost with a deletion of an entire fact compared to an update of a single attribute value.
%For relation schema $\rel{Airport}$ in Example~\ref{eg:running}, if we apply $\del{t_5}{D_1}$ on Figure~\ref{fig:noisy-1}, we will get another database instance $D_1'$ with tuples $t_1, \cdots, t_4$ from $D_1$. Similarly, if we have a fact $f_5$ = {\tt KNQX, Medium airport, Naval Air Station Key West/Boca Chica Field, Am, US, Key West} with a tuple identifier $t_5$, then  $\ins{f_5}{D_1'} = D_1$. \red{can we use $t_5$?} As an example of attribute update, $\upd{t_5.{\tt Continent}}{{\tt NAm}}{D_1}$ gives $D_2$ in Figure~\ref{fig:noisy-2} that changes the {\tt Continent} attribute of $t_5$ from {\tt Am} to {\tt NAm}. 
\end{example}


==> preliminaries__Benny_Kimelfeld_s_conflicted_copy_2020-09-22_1_.tex <==
\section{Preliminaries}\label{sec:prelim}
We first give the basic terminology and concepts.

\subpagraph*{Relational Model}
A \e{relation signature} is a sequence $\alpha=(A_1,\dots,A_k)$ of
distinct \e{attributes} $A_i$, where $k$ is the \e{arity} of
$\alpha$. A \e{relational schema} (or just \e{schema} for short)
$\scs$ has a finite set of \e{relation symbols} $R$, each associated with a signature that we denote by $\sig(R)$.
If $\sig(R)$ has arity $k$, then we say that $R$ is $k$-ary.  A
\e{fact} $f$ over $\scs$ is an expression of the form
$R(c_1,\dots,c_k)$, where $R$ is a $k$-ary relation symbol of $\scs$,
and $c_1$,\dots, $c_k$ are \e{values}. When $\scs$ is irrelevant or
clear from the context, we may call a fact over $\scs$ simply a
\e{fact}.  If $f=R(c_1,\dots,c_k)$ is a fact and
$\sig(R)=(A_1,\dots,A_k)$, then we refer to the value $c_i$ as $f.A_i$.

%(where $i=1,\dots,k$).

A \e{database} $D$ over $\scs$ is a mapping from a finite set
$\tids(D)$ of \e{record identifiers} to facts over $\scs$. The set of all databases over a schema
$\scs$ is denoted by $\dbs(\scs)$.  We denote by $D[i]$ the fact that
$D$ maps to the identifier $i$. A database $D$ is a \e{subset} of a
database $E_1$, denoted $D\subseteq E_1$, if
$\tids(D)\subseteq\tids(E_1)$ and $D[i]=E_1[i]$ for all $i\in\tids(D)$.

An \e{integrity constraint} is a first-order sentence over $\scs$. A
database $D$ satisfies a set $\Sigma$ of integrity constraints,
denoted $D\models\Sigma$, if $D$ satisfies every constraint
$\sigma\in\Sigma$. If $\Sigma$ and $\Sigma'$ are sets of integrity
constraints, then we write $\Sigma\models\Sigma'$ to denote that
$\Sigma$ \e{entails} $\Sigma'$; that is, every database that satisfies
$\Sigma$ also satisfies $\Sigma'$. We also write $\Sigma\equiv\Sigma'$
to denote that $\Sigma$ and $\Sigma'$ are \e{equivalent}, that is,
$\Sigma\models\Sigma'$ and $\Sigma'\models\Sigma$. By a \e{constraint
  system} we refer to a class $\C$ of integrity constraints (e.g., the
class of all functional dependencies).

As a special case, a \e{Functional Dependency} (FD) $R:X\rightarrow Y$, where $R$ is a relation symbol and $X,Y\subseteq\sig(R)$, states that every two facts that agree on (i.e., have equal values in) every attribute in $X$ should also agree on every attribute in $Y$. The more general \e{Equality Generating Dependency} (EGD) has the form $$\forall\vec x\left[\varphi_1(\vec x)\wedge\dots\wedge\varphi_k(\vec x)\rightarrow (y_1=y_2)\right]$$ where each $\varphi_j(\vec x)$ is an atomic formula over the schema and $y_1$ and $y_2$ are variables in $\vec x$. Finally, a \e{Denial Constraint} (DC) has the form $$\forall\vec x\neg\left[\varphi_1(\vec x)\wedge\dots\wedge\varphi_k(\vec x)\wedge\psi(\vec x)\right]$$ where each $\varphi_j(\vec x)$ is an atomic formula and $\psi(\vec x)$ is a conjunction of atomic comparisons over $\vec x$.

\begin{example}\label{eg:db-constraints}
%\ester{I am not sure that we need this example}
In Figure~\ref{fig:running}, we have a single 5-ary relation symbol $\rel{Airport}$. All databases have five facts with $\tids(D) = \{f_1, \cdots, f_5\}$. The set of integrity constraints $\Sigma$, which consists of two FDs, is given in Example~\ref{eg:running}.  
\end{example}

\subsection*{Repair Systems}
Let $\scs$ be a schema. A \e{repairing operation} (or just
\e{operation}) $o$ transforms a database $D$ over $\scs$ into another
database $o(D)$ over $\scs$, that is,
$o:\dbs(\scs)\rightarrow\dbs(\scs)$. An example is \e{tuple deletion},
denoted $\del{i}{\cdot}$, parameterized by a tuple identifier $i$ and
applicable to a database $D$ if $i\in\tids(D)$; the result
$\del{i}{D}$ is obtained from $D$ by deleting the tuple identifier $i$
(along with the corresponding fact $D[i]$).  Another example is
\e{tuple insertion}, denoted $\ins{f}{\cdot}$, parameterized by a fact
$f$; the result $\ins{f}{D}$ is obtained from $D$ by adding $f$ with a
new tuple identifier. (For convenience, this is the minimal integer
$i$ such that $i\notin\tids(D)$.) A third example is \e{attribute
  update}, denoted $\upd{i.A}{c}{\cdot}$, parameterized by a tuple
identifier $i$, an attribute $A$, and a value $c$, and applicable to
$D$ if $i\in\tids(D)$ and $A$ is an attribute of the fact $D[i]$; the
result $\upd{i.A}{c}{D}$ is obtained from $D$ by setting the value
$D[i].A$ to $c$. By convention, if $o$ is not applicable to $D$, then
it keeps $D$ intact, that is, $o(D)=D$.

A \e{repair system} (over a schema $\scs$) is a collection of
repairing operations with an associated \e{cost} of applying to a
given database. For example, a smaller change of value might be less
costly than a greater one~\cite{DBLP:conf/lid/GardeziBK11}, and some
facts might be more costly than others to
delete~\cite{DBLP:conf/icdt/LopatenkoB07,DBLP:conf/pods/LivshitsKR18}
or
update~\cite{DBLP:conf/icdt/KolahiL09,DBLP:conf/pods/LivshitsKR18,DBLP:journals/is/BertossiBFL08};
changing a person's zip code might be less costly than changing the
person's country, which, in turn, might be less costly than deleting
the entire person's record.  Formally, a repair system $\R$ is a pair
$(O,\kappa)$ where $O$ is a set of operations and
$\kappa:O\times\dbs(\scs)\ra[0,\infty)$ is a cost function that
assigns the cost $\kappa(o,D)$ to applying $o$ to $D$. We require that
$\kappa(o,D)=0$ if and only if $D=o(D)$; that is, the cost is nonzero
when, and only when, an actual change occurs.

For a repair system $\R$, we denote by $\R\str=(O\str,\kappa\str)$ the repair system 
of all \e{sequences} of operations from $\R$, where the cost
of a sequence is the sum of costs of the individual operations
thereof. 
\textforlongversion{
Formally, for $\R=(O,\kappa)$, the repair system $\R\str$ is
$(O\str,\kappa\str)$, where $O\str$ consists of all compositions
$o=o_m\circ\dots\circ o_1$, with $o_j\in O$ for all $j=1,\dots,m$,
defined inductively by $o_m\circ\dots\circ
o_1(D)=o_m(o_{m-1}\circ\dots\circ o_1(D))$ and
$\kappa\str(o_m\circ\dots\circ
o_1,D)=\kappa(o_m,o_{m-1}\circ\dots\circ
o_1(D))+\kappa\str(o_{m-1}\circ\dots\circ o_1,D)$.
}
Let $\C$ be a constraint system and $\R$ a repair system. We say that
$\C$ is \e{realizable by} $\R$ if it is always possible to make a
database satisfy the constraints of $\C$ by repeatedly applying operations
from $\R$. Formally, $\C$ is realizable by $\R$ if for every database
$D$ and a finite set $\Sigma\subseteq\C$ there is a sequence $o$ in
$\R\str$ such that $o(D)\models\Sigma$.  An example of $\C$ is the
system $\Cfd$ of all FDs $R:X\ra Y$.
%, where $R$ is a relational symbol
%and $X,Y\subseteq\sig(R)$, stating that every two facts that agree on
%(i.e., have equal values in) every attribute in $X$ also agree on
%every attribute in $Y$.  
An example of $\R$ is the \e{subset} system,
denoted $\R_\subseteq$, where $O$ is the set of all tuple deletions
(hence, the result is always a subset of the original database), and
$\kappa$ is determined by a special \e{cost} attribute,
$\kappa(\del{i}{D})=D[i].\mathtt{cost}$, if a cost attribute exists, and otherwise,
$\kappa(\del{i}{D})=1$ (every tuple has unit cost for  deletion). Observe that $\R_\subseteq$ realizes $\C$,
since the latter consists of anti-monotonic constraints.

\begin{example}\label{eg:repair}
The database $D_1$ of Figure~\ref{fig:noisy-1} may be obtained from $D_0$ by applying the following sequence of attribute updates (here, we assume that the identifier of a fact $f_i$ is $i$):
{\small
\begin{align*}
    &E_1=\upd{2.\att{Continent}}{\val{Am}}{D_0}\\
    &E_2=\upd{2.\att{Country}}{\val{USA}}{E_1}\\
    &E_3=\upd{4.\att{Country}}{\val{USA}}{E_2}\\
    &D_1=\upd{5.\att{Continent}}{\val{Am}}{E_3}
\end{align*}
}
If we consider tuple deletions (i.e., the repair system $\R_\subseteq$), we may obtain $D_1$ from $D_0$ by applying the following sequence of operations:
{\small
\begin{align*}
    &E_1=\del{2}{D_0}\,\,\,\,\,\,\,\,\,\,\,\,
    E_2=\ins{f_2}{E_1}\\
    &E_3=\del{4}{E_2}\,\,\,\,\,\,\,\,\,\,\,\,
    E_4=\ins{f_4}{E_3}\\
    &E_5=\del{5}{E_4}\,\,\,\,\,\,\,\,\,\,\,\,
    D_1=\ins{f_5}{E_5}
\end{align*}
}
where $f_2,f_4$ and $f_5$ are the facts of the database $D_1$. We may also assign a cost to each one of these operations. For example, if both tuple deletions and attribute updates are allowed, we may associate a higher cost with a deletion of an entire fact compared to an update of a single attribute value.
%For relation schema $\rel{Airport}$ in Example~\ref{eg:running}, if we apply $\del{t_5}{D_1}$ on Figure~\ref{fig:noisy-1}, we will get another database instance $D_1'$ with tuples $t_1, \cdots, t_4$ from $D_1$. Similarly, if we have a fact $f_5$ = {\tt KNQX, Medium airport, Naval Air Station Key West/Boca Chica Field, Am, US, Key West} with a tuple identifier $t_5$, then  $\ins{f_5}{D_1'} = D_1$. \red{can we use $t_5$?} As an example of attribute update, $\upd{t_5.{\tt Continent}}{{\tt NAm}}{D_1}$ gives $D_2$ in Figure~\ref{fig:noisy-2} that changes the {\tt Continent} attribute of $t_5$ from {\tt Am} to {\tt NAm}. 
\end{example}


==> response.tex <==
%\begin{center}
\cut{
{\large \textbf{Properties of Inconsistency Measures for Databases}}
\vskip1em
%\def\thefootnote{\fnsymbol{footnote}}

%\def\au#1
\textbf{Anonymous Author(s)}


\vskip3em



{\underline{\large Cover Letter for Revision}}\vskip3em
}
%\end{center}

\begin{center}
    
{\large{\textbf{Properties of Inconsistency Measures for Databases}}}\\
\vskip1em
\textbf{Anonymous Author(s)}\\
\vskip2em
\underline{\large{Cover Letter for Revision}}
\vskip2em
\end{center}

\noindent 
We are very grateful for the hard work and valuable comments and
suggestions of the reviewers. We have revised our paper by
incorporating the comments and suggestions. %In particular, we
%completely rewrote the complexity section in the preliminaries
%(Section 2.4), and revised the relevant results and proofs
%accordingly.  Of course, 
We have fixed the indicated
errors, added clarifications wherever their need has been raised
by the reviewers, re-organized the paper, and significantly extended our experimental evaluation. We believe that the revised paper is a considerable
improvement compared to the original submission, and we highly
appreciate the serious reviewers for that.  %Due to a lack of space, we
%have moved the proofs of Theorem 5.14 and 5.15 to an online
%appendix. 
We have marked the significant changes in the paper with different font colors:
\begin{itemize}
    \item \revone{violet} for reviewer 1, 
    \item \revtwo{magenta} for reviewer 2, 
    \item \revthree{blue} for reviewer 3,
    \item 
    \mrev{red} for meta reviewer's comment, common comments, and general improvements in presentation.
\end{itemize}    
    
To make room for new additions, we had to move some proofs to the (anonymous) full version of the paper \cite{extended}.\\

Please note that the old Sections~5 (Computational Complexity) and 6 (Rational and Tractable Measures) have been merged into the new Section~\ref{sec:rational}; therefore, the old Sections~7 and 8 now appear as Sections~\ref{sec:experiments} and \ref{sec:conclusions}.\\

Please see below our responses to the
specific comments with pointers to the changes in the paper.

\section*{Meta-review}
\begin{reviewcomment}
1. One of the major points that was discussed was the \underline{narrow scope of the contributions}. The reviewers are concerned that the narrowness of scope will translate to small impact and interest. They hope that the revision will alleviate this issue to some extend. 
\end{reviewcomment}
\begin{authorreply}
 \rmrev{
 We have clarified the scope of the contributions both by updating the presentation as well as by adding new experiments. 
 \begin{enumerate}
  \item  We have clarified (e.g., in \textbf{Section~\ref{sec:introduction} and at the end of Section~\ref{sec:rational}}) that a chosen measure of inconsistency can be applied with \emph{any} repair system that works with a set of integrity constraints, and these measures {\em do not} restrict the repair operations (e.g., tuple deletions vs. value updates) that a repair system allows or applies. It is just that we provide theoretical guarantees in terms of some repairing operations and integrity constraints (e.g., for $\Imr, \Ilmr$, continuity and progression are guaranteed only for deletion operations, and could be violated otherwise). To complement these theoretical results, and to show broader applicability of the inconsistency measures, we have significantly extended the empirical evaluation that also includes {\em updates} of attribute values. 
 \item As the reviewers suggested, we have illustrated properties of the existing measures and suitability of the new measure with new experiments with respect to a case study using the HoloClean repair system \cite{DBLP:journals/pvldb/RekatsinasCIR17}. It can be seen in the new Figure~\ref{fig:holoclean} that $\Imr$ and $\Ilmr$ exhibit desired smoothness and progress compared to other measures as a noisy dataset becomes more clean step by step by HoloClean {\bf (Section~\ref{sec:exp:holoclean})}.
 \item As Reviewer 3 suggested, we have clarified the scope of the paper, that focuses on the case when the inconsistency is defined in terms of a given set of integrity constraints {\bf (Section~\ref{sec:introduction})}.
  \end{enumerate}
  Please also see our detailed responses to \textbf{Reviewer1-author feedback} or \textbf{Reviewer2-O2}, and to \textbf{Reviewer3-O1} for additional details on the scope and impact of our work.
 }

\end{authorreply}
\begin{reviewcomment}
2. They also propose improvements in the \underline{experiments}, and expect to see clarifications given in the author incorporated into the revised submission.
\end{reviewcomment}
\begin{authorreply}
 \rmrev{
We have added several new experiments and further discussions  as suggested by the reviewers \textbf{(Section~\ref{sec:experiments})}:
\begin{enumerate}
    \item We discuss \textbf{two `noise generation' algorithms}: (a) as used earlier, \textbf{CONoise (Constrained-Oriented Noise)}, which introduces random violations of a randomly chosen constraint, and (b) a new one, \textbf{RNoise (Random Noise)}, which randomly \underline{updates} the value of a randomly-chosen cell either to another value from the active domain or to a typo, and can control the level of noise in the dataset (by parameter $\alpha$) and the skewness in the dataset (by parameter $\beta$ in the Zipfian distribution) \textbf{(Section~\ref{sec:expt-setup})}.
    \item Using the above two noise generation algorithms, we evaluate our methods in terms of \textbf{both value updates and deletion-based repairs, overlapping constraints, data skew, and noise level} in the database \textbf{(Section~\ref{sec:exp:behavior})}. We could not illustrate some graphs varying data skew (the parameter $\beta$ in the Zipfian distribution) due to space constraints. Those graphs showed similar behavior as explained in text. They can be found in the anonymous full version of the paper \cite{extended}. \sudeepa{attach at the end of the response letter?}
    \item We added a new case study with a state-of-the-art data repair system \textbf{HoloClean} \cite{DBLP:journals/pvldb/RekatsinasCIR17} that we treat as a black box. We use the `Hospitals' dataset where HoloClean has been shown to be highly accurate. Since HoloClean provides one-shot cleaning (and uses soft rules), we add a single DC at a time to the constraints set to simulate a cleaning pipeline (using 15 DCs and varying their orders). We show that $\Imr$ and $\Ilmr$ exhibit smoothness and steady progress compared to other methods as desired \textbf{(Section~\ref{sec:exp:holoclean} and Figure~\ref{fig:holoclean})}. 
    \item We added experiments to show \textbf{scalability} in terms of larger datasets varying the number of tuples going up to 1 million tuples \textbf{(Section~\ref{sec:exp:runningtime})}.
    \item We added details about all the datasets used in our experiments including the numbers of tuples, attributes, and DCs, example constraints, and amount of overlap in the constraints \textbf{(Figure~\ref{fig:datasets})}.
    \item We added details on the implementations of the measures \textbf{(Section~\ref{sec:expt-setup})}.
\end{enumerate}
}
\end{authorreply}
\begin{reviewcomment}
3. \underline{Required Changes:}
The reviewers have listed their requirements for the revision in their responses to Q13. The authors need to address these comments convincingly for the paper to be accepted.
\end{reviewcomment}
\begin{authorreply}
 \rmrev{
We have addressed all required changes mentioned by all three reviewers. Please see our responses and pointers to the changes below highlighted with a different font color. 
}
\end{authorreply}
\section*{Reviewer 1}

\begin{reviewcomment}
O1: In Section 4, there are some exceptions to properties based on the type of integrity constraint.
I would have liked to see a more systematic discussion for each property to a standard set of integrity constraints; thereby making it explicit how each property holds (or not) for each type of constraint.
 \end{reviewcomment}
\begin{authorreply}
  \rrevone{ Indeed, this distinction needed better clarity. We have added
    clarifications to the text in  \textbf{Section~\ref{sec:postulates}}.  We have also changed
    \textbf{Table~\ref{table:postulates}} so that it now explicitly
    separates between FDs and DCs and summarizes which properties
    hold for FDs and which hold for DCs (e.g., ``\checkmark/\xmark''
    means that the property holds for FDs but not for the general
    class of DCs). }

 % \sudeepa{TODO: See if  should be explained in text too}
\end{authorreply}

\begin{reviewcomment}
O2:  To allow users to apply these metrics, I would recommend providing algorithmic details of how to efficiently compute the measures, i.e., $I_R$, $I_R^{lin}$, $I_{MC}$. They are alluded to in Sec. 7.1, but no further details or pseudocode is given.
 \end{reviewcomment}
\begin{authorreply}
  \rrevone{ We have added more details about the implementation of the measures. \textbf{Please see ``Implementation Details'' in Section~\ref{sec:expt-setup}.} We have also highlighted the parts where the complexity of different measures is discussed with paragraph headings. \textbf{Please see Section~\ref{sec:complexity}.} Additional experiments and discussions on scalability of different measures have been added to \textbf{Section~\ref{sec:exp:runningtime}.}
  
  We
    note, however, that the focus of our work here is \e{not} on how
    to efficiently compute the measures, but rather on formally
    expressing and establishing their pros and cons, including their
    rationality and computational complexity. For example, $\Imc$ is
    a bad choice since it violates almost all of the properties and,
    in addition, is inherently intractable. In particular, optimizing
    $\Imc$ is really outside the scope of the paper; in fact, its
    empirical inefficiency strengthens the theoretical insights about
    it.  For similar reasons, our implementation of the tractable
    measures is rather simple (e.g., a direct translation into SQL and then
    ILP/LP as now discussed in Section~\ref{sec:expt-setup}).
}    
%    \sudeepa{TODO: check if the color of this implementation paragraph should change to revone} 

\end{authorreply}

\begin{reviewcomment}
O3: Evaluation is done on a very small data size. Experimental configuration details are not given: what are the set of DCs?
 \end{reviewcomment}
\begin{authorreply}
  \rrevone{ We thank the reviewer for encouraging us to target larger
    datasets. We are quite satisfied with the outcome.  We have
    reapplied all of the experiments on considerably larger
    datasets. We now use datasets with 10K tuples for the
    measure-behavior experiments (\textbf{Section~\ref{sec:exp:behavior}}), and we experiment with larger
    datasets (up to 1M tuples) for the running-time experiments (\textbf{Section~\ref{sec:exp:runningtime}}). We
    have also added more details about the datasets and constraints of
    the experiments. See \textbf{Figure~\ref{fig:datasets}}. The full datasets and constraint sets (as well as our implementation) can be found in~\url{https://drive.google.com/drive/folders/1jdyCMNYpQO0FxOdvya6cRfJz_iakrRsB?usp=sharing}.
}
%\sudeepa{Check if we should add a paragraph on datasets used--   probably not needed.}  }

\end{authorreply}

\begin{reviewcomment}
O4: The evaluation was rather limiting. Given these are inconsistency measures, the evaluation does not study the
impact of varying error rates, overlapping dependencies to study interaction between errors, and the impact of different data skew.
 \end{reviewcomment}
\begin{authorreply}
  \rrevone{Please see the details of the extended experiments section in our response to the  \textbf{Meta-reviewer's second comment on experiments}.  In particular, in addition to the aforementioned increase of number of tuples, we
    have also considerably extended our experimental evaluation. In
    particular, we have conducted experiments with several different
    parameters to test the effect of \textbf{error rate}, \textbf{data
      skewness}, and \textbf{error type} (typo or wrong value) on the
    measures. 
\begin{enumerate}
\item \textbf{Error rates and types:} We have added a new method for
  introducing noise where we modify cells in the dataset by either
  changing the value to a new value from the active domain of the
  attribute or a typo. This method allows us to control both the error rate (the more values we change, the higher the error rate is), as well as the type of errors, and we use different parameters to test the impact of these parameters on the behavior of the measures. \textbf{Please see Section~\ref{sec:exp:behavior}.}
\item \textbf{Overlapping dependencies:} We have added a chart to \textbf{Figure~\ref{fig:datasets}} that depicts the level of attribute overlapping of the constraints for each dataset. It shows that the sets of constraints that we use have different levels of overlapping. The results are discussed in \textbf{Section~\ref{sec:exp:behavior}.}
  %We also do not see any clear correlation between overlapping dependencies and the behavior of the measures. We showed that the constraint sets that we use have different levels of overlapping, but the measures behave similarly on all of them. \textbf{Please see Section~\ref{} and Figure~\ref{}.}
    \item \textbf{Data skew:} To evaluate data skew, we use the Zipfian distribution for the choice of values from the domain. We use different parameters to test the effect of data skewness on the behavior of the measures. \textbf{Please see Section~\ref{sec:exp:behavior}.} 
    \end{enumerate}
     The conclusion is that the behavior of the measures is
    rather robust to these parameters, as we did not observe any
    dramatic change in reaction to differences in the parameter
    values. See \textbf{Section~\ref{sec:experiments}}.

    In addition, we performed new experiments over the HoloClean
    system~\cite{DBLP:journals/pvldb/RekatsinasCIR17}, where we
    provided it with  increasingly larger sets of constraints and applied
    the measures after each cleaning application. Please see
    \textbf{Section~\ref{sec:exp:holoclean}}.

    Finally, we note that some of the results (e.g., varying parameters for data skew, where we observed comparable behavior) are provided in the extended
    version of the paper~\cite{extended} due to lack of space.  }
  
%\ester{We can also say something about the HoloClean experiment. Due to lack of space, some of the results are given only in the extended version of the paper~\cite{extended}.}
%\sudeepa{@Ester: could you add the missing results at the end of the cover letter? People may not check the full version.}
\end{authorreply}

\textbf{Response to author feedback:}
\begin{reviewcomment}
Thank you for your clarifications. The evaluation needs to be strengthened significantly to demonstrate the utility of the metric, its sensitivity to various parameters, and to show potential impact.
 \end{reviewcomment}
\begin{authorreply}
\rrevone{
Please see the preceding answers to the comments, and also our responses to the other reviewers' comments and meta-reviewer's high-level comments for the extended evaluations including sensitivity to various parameters and impact of this work.}

\rrevone{In particular, the utility and potential impact of our work can be briefly described as follows: our original submission’s focus was on the idea of a framework for inconsistency measures with a set of desired properties motivated by inconsistency measures in knowledge bases, where we showed theoretical properties (for certain repair systems and integrity constraints) and proof-of-concepts through a set of experiments. Following the reviewers' thoughtful suggestions,  in the revised version, we have expanded the experiments section significantly to illustrate  (1) how the inconsistency measures help track progress  in a repair system when their desired properties are satisfied (e.g., by showing smooth progress and avoiding jumps and jitters), (2) the applicability of inconsistency measures goes beyond the settings for which theoretical results have been proved (e.g., while the majority of our theoretical results are in terms of tuple deletions, inconsistency measures are equally useful when value updates are used for repair), and (3) usefulness of inconsistency measures for practical repair systems using a state-of-the art repair system (HoloClean) as a block box.}

\rrevone{To the best of our knowledge, no prior works have (i) studied such properties in the context of repair systems, (ii) showed theoretical properties and complexity results for relational databases and integrity constraints (FDs, EGDs, DCs), (iii) proposed our new measure $\Ilmr$ that is both rational and tractable for tuple deletions and works well in practice for other repair systems involving updates, and (iv) conducted a thorough experimental evaluations for relational databases and integrity constraints. }

\rrevone{We have emphasized the impact and utility throughout the revised paper, especially in the updated introduction and related work \textbf{(Section~\ref{sec:introduction})}.}
%,  in the following way and showed that it worked in the following cleaning scenario (optimization/scalability/implementation/hashing/reduce vars to send to LP solver.

%\sudeepa{Add impact using HoloClean expts.}
\sudeepa{@all: Please check the impact statement -- added from the google doc based on our discussions. }
\end{authorreply}

\textbf{Required changes for revision:}
\begin{reviewcomment}
O1-O4.
 \end{reviewcomment}
\begin{authorreply}
\rrevone{
All of these have been addressed, as we explained in the answers to
the comments themselves.  We believe that our submission has
considerably improved due to these comments, and we are grateful for that.
}
\end{authorreply}

\section*{Reviewer 2}

\begin{reviewcomment}
O1: The novelty of the approach is not clearly explained with key differentiation elements, given the literature on the topic (e.g., \url{http://www.mthimm.de/pub/2017/Thimm_2017.pdf}).
 \end{reviewcomment}
\begin{authorreply}
  \rrevtwo{ We have extended the discussion of the connection to
    related work in the introduction
    \textbf{(Section~\ref{sec:introduction}, please see ``Other related work'')}. Specifically, in comparison with
    the work of Thimm~\cite{DBLP:journals/ki/Thimm17} on knowledge
    bases, our contributions are as follows
\begin{itemize}
\item We devise specific properties that are tailored to data repairs
  and their impact on the measures. To the best of our knowledge,
  properties in the context of a repair system have not been studied
  in the past, and we believe that inconsistency measures should be
  sensitive to the repair system (as we explain throughout the paper).
\item We investigate the computational complexity of the measures and
  establish novel results (that, in particular, are not mentioned in
  the referenced paper).
\item We show how the theoretical analysis leads to the selection of a
  new measure of inconsistency, namely $\Ilmr$. This is a novel
  measure, which is motivated by both rationality and efficiency, and
  such that has been neither proposed nor justified in past research.
%
\item We conduct the empirical evaluation (which is considerably more
  thorough in this revision than in the original submission) on the
  behavior of the measures in a repairing process, which goes beyond the settings described in our theoretical results (e.g., while our theoretical results are mostly for tuple deletions, our empirical results show that the proposed measures $\Imr, \Ilmr$ perform well also for repair systems with value updates). As far as we know,
  this work is the first to conduct such an evaluation on
  inconsistency measures.
  \end{itemize}
%Please see the highlighted text in \textbf{Section~\ref{sec:introduction}}.
}
\end{authorreply}

\begin{reviewcomment}
O2: The impact of the properties and new measure could be demonstrated "in action" with respect to the cost of repairing. More specifically, the actionability and utility of the proposed approach seem to be very narrow and the impact of the proposed metric is not clear.
 \end{reviewcomment}
\begin{authorreply}
\rrevtwo{(The following response is the same as that to Reviewer1-author feedback, which we repeat here for easy access.)} 

\rrevtwo{
Please see the preceding answers to the comments, and also our responses to the other reviewers' comments and meta-reviewer's high-level comments for the extended evaluations including sensitivity to various parameters and impact of this work.}

\rrevtwo{In particular, the utility and potential impact of our work can be briefly described as follows: Our original submission’s focus was on the idea of a framework for inconsistency measures with a set of desired properties motivated by inconsistency measures in knowledge bases, where we showed theoretical properties (for certain repair systems and integrity constraints) and proof-of-concepts through a set of experiments. Following the reviewers' thoughtful suggestions,  in the revised version, we have expanded the experiments section significantly to illustrate  (1) how the inconsistency measures help track progress  w.r.t. a repair system when their desired properties are satisfied (e.g., by showing smooth progress and avoiding jumps and jitters), (2) the applicability of inconsistency measures go beyond the settings for which theoretical results have been proved (e.g., while the majority of our theoretical results are in terms of tuple deletions, inconsistency measures are equally useful when value updates are used for repair), and (3) usefulness of inconsistency measures for practical repair systems using a state-of-the art repair system (HoloClean) as a block box.}

\rrevtwo{To the best of our knowledge, no prior works have (i) studied such properties in the context of repair systems, (ii) showed theoretical properties and complexity results for relational databases and integrity constraints (FDs, EGDs, DCs), (iii) proposed our new measure $\Ilmr$ that is both rational and tractable for tuple deletion and works well in practice for other repair systems involving updates, and (iv) conducted a thorough experimental evaluations for relational databases and integrity constraints. }

\rrevtwo{We have emphasized the impact and utility throughout the revised paper, especially in the updated introduction and related work \textbf{(Section~\ref{sec:introduction})}.}

\sudeepa{@all: I replaced the previous reponse (cut below) following the one we discussed in the meeting as it appears more direct to me. Please check.}

\cut{
  \rrevtwo{ We believe that the principles and analysis that we
    establish in the paper constitute a significant progress in
    addressing the challenge of measuring inconsistency in database
    repairing (and more generally cleaning and quality-management)
    systems. Moreover, we believe that this challenge is fundamental,
    practical, and highly common.

    The above said, we accept the statement that the experiments
    should be more thorough than the original version, and indeed, we
    extended our empirical study significantly. In addition to
    considering bigger and more varied settings, we have performed new
    experiments over the HoloClean
    system~\cite{DBLP:journals/pvldb/RekatsinasCIR17}. As we
    explain in our reply to Reviewer~1, the experiment has been
    conducted by providing HoloClean with increasingly larger sets of
    constraints and applying the measures after each cleaning
    application. We believe that our current experimental study
    delivers a strong indication of the usefulness and potential
    impact of our work and paper. Please see
    \textbf{Section~\ref{sec:exp:holoclean}}.}
}    
    
    

%\ester{I am not sure what he means, but I guess we can say something about the fact that we have conducted experiments using two different methods for introducing noise, with different distributions and parameters, and we also tested it on HoloClean, and we obtain surprisingly good results for some of the measures.}\\
%\sudeepa{We need to add the holoclean discussion}
\end{authorreply}

\begin{reviewcomment}
O3: The experimental evaluation does not provide enough details on the setup and methodology to properly evaluate the quality of the results and the benefit of the new and existing measures (e.g., the number of violations injected, the distribution of the violations and also the repairs, the number of newly introduced violations due to repairs, etc.). As claimed by the authors, the focus is not to compute the measures in the most efficient way, so Table 2 does not show the benefit of the newly proposed measure, but Figure 1 (normalized value of the metrics) and its interpretation does not show the benefit either.
 \end{reviewcomment}
\begin{authorreply}
  \rrevtwo{Please see the details of the extended experiments section in our response to the  \textbf{Meta-reviewer's second comment on experiments} and to \textbf{Reviewer1-O4}.
  We have added details on how to vary distributions of violations, setup, and methodology in \textbf{Section~\ref{sec:experiments}}.
  }  

\sudeepa{Unlike the above comment, I could not copy paste as we have not addressed the part in parentheses yet like distribution or repairs(??)}
\cut{  \rrevtwo{ Please see our reply to Comment O4 of Reviewer~1. In
    addition to extending the experimental study, we have also added
    missing details on the (extended) experiments in
    \textbf{Section~\ref{sec:experiments}}. }
    }
  %\ester{We have added more details
   % about the datasets, constraints, implementation and algorithms
   % that we use. We have also conducted new experiments with varying
   % error rates and distributions of the data.}
\end{authorreply}

\begin{reviewcomment}
O4: The paper is hard to read due to its non-linear structure and
organization:
\begin{enumerate}
  \item The illustrative example (and Figure 1) cannot be understood
    without reading Section 3 first; in other words, the reader has to
    interrupt the reading of the introduction to read Section 3.
    \item To understand the proof of Proposition 3, the reader has to
      read Proposition 4 first.
      \item The properties of inconsistency measures are divided
        unnecessarily in two sections: Section 4 and Section 6.
        \end{enumerate}
 \end{reviewcomment}
\begin{authorreply}
\rrevtwo{
Thank you for the suggestions. We have rewritten and reorganized various parts of the paper. In particular, 
\begin{enumerate}
    \item We have made significant changes to the Introduction to
      incorporate the reviewer comments. 
      Table~\ref{tab:running_measures} (that discusses values of
      different measures on the two noisy tables) and the discussion
      on the values of the specific measures have been moved
     to Section~\ref{sec:measure}. Hence, the illustration and numbers
     appear only after the measures are formally introduced. \textbf{Please see  Example~\ref{eg:running} and  Section~\ref{sec:measure}}.
     \item We have reorganized Section~\ref{sec:measure} (inconsistency measures) to discuss the measures ($\Id, \Imi, \Ip, \Imc$) from the KR literature first and then the repair-system based measure $\I_R$. As mentioned above, we now illustrate the measures on the databases of our running example in this section (rather than the Introduction). \textbf{Please see Section~\ref{sec:measure} and Table~\ref{tab:running_measures}.} 
    \item We have also \textbf{reorganized Section~\ref{sec:postulates}} and
      resolved the issue with the order of the propositions.
    \item 
    %In our viewpoint, the organization of Sections~\ref{sec:postulates}--\ref{sec:rational} supports the  following storyline, which we find both interesting and clear.
    We have \textbf{merged old Sections~5 and 6 into the new Section~\ref{sec:rational}}. The new organization of the sections support the following storyline.
      \begin{itemize}
        \item Section~\ref{sec:postulates} describes the desired properties/postulates and illustrates them on the measures discussed in the previous Section~\ref{sec:measure}. We show that all the measures, except one ($\Imr$) violate at least one of the properties.
        \item Then, the discussion in Section~\ref{sec:complexity} establishes that the only rational measure is intractable in most cases; hence, all the existing measures either lack tractability ($\Imr$) or at least one of the desired properties (all other measures).
        \item This build up a need for new measures beyond those mentioned, that are both rational and tractable. This need is addressed in Section~\ref{sec:lmr}, where we devise a polynomial-time measure that satisfies the properties (namely $\Ilmr$) for the special case where the repairing operations are tuple deletions. We also show, in Section~\ref{sec:more-general}, that devising such measures for more general repair systems is a challenging task.
        %introduces the measure properties and discusses the corresponding behavior of different existing measures.
          %\item Section~\ref{sec:complexity} studies the complexity of the existing measures.
          %\item Therefore, in the next section (new Section~\ref{sec:rational}, old Section~6), we ask the question if it is possible to achieve both rationality in terms of all the desired measures as well as tractability. We show in Section~\ref{sec:lmr} that it is indeed possible for a repair system involving only tuple deletion by introducing our new measure $\Ilmr$. However, we also show in Section~\ref{sec:more-general} that such measures in general may not be achievable.
          %\item Together, Sections~\ref{sec:postulates} and~~\ref{sec:complexity} build up a need for new measures beyond those mentioned, since the rational measures are intractable and the tractable measures are irrational. This need is addressed in Section~\ref{sec:rational} where, in particular, we devise a polynomial-time measure that satisfies the properties (namely $\Ilmr$).
          \end{itemize}
      \item We have \textbf{added a new organization/roadmap paragraph} at the end of the introduction \textbf{(Section~\ref{sec:introduction})} to clarify the organization of the paper.  
\end{enumerate}
}
%      \benny{Maybe we should add something to the Organization part of
     %   the Introduction? (Just a thought so that we can say that we
      %  did something to address the comment.)}
      %  \sudeepa{done.}
\end{authorreply}

\textbf{Additional Remarks:~}

\begin{reviewcomment}
D1. Please reorganize the paper
 \end{reviewcomment}
 \begin{authorreply}
 \rrevtwo{
     Done, \textbf{please see our response to Reviewer2-O4 above}.
%\ester{Done.}
}
\end{authorreply}


\begin{reviewcomment}
D2. Expand the experimental section to include detailed setup and discussions; add various configurations, data sets and repairing strategies to demonstrate the added-value of the contribution
 \end{reviewcomment}
 \begin{authorreply}
\rrevtwo{     Done, \textbf{please see our response to Reviewer2-O3 above}.}
%\ester{done}

\end{authorreply}

\begin{reviewcomment}
D3. Motivate the usefulness of the contribution wrt the cost repairing and the choice of repairing strategy from the introduction, through the examples, to the experiments.
 \end{reviewcomment}
 \begin{authorreply}
   \rrevtwo{
          Done, \textbf{please see our responses to Reviewer2-O2 and Reviewer2-O1 above}.
     %We have made a significant revision the paper, and particularly the Introduction and experimental study, as we explained in the preceding items. We believe that the current version makes the case in a much stronger way, and we hope that it satisfies the intention of the reviewer.
%\ester{not sure what it means}
}
\sudeepa{Not sure if I follow ``cost repairing'' part of the comment -- @all: any idea?}
\end{authorreply}
 
\textbf{Response to author feedback:}
\begin{reviewcomment}
I thank the authors for addressing my comments. However, the sensitivity and utility of the proposed measures are not clearly defended and demonstrated. The setting and scope of the contribution remain very narrow. The impact of the properties and the new measure could be demonstrated with experiments showing the utility and benefit of the measure with respect to the cost of repairing for example.
 \end{reviewcomment}
 \begin{authorreply}
\rrevtwo{
  We have added details and experiments on the sensitivity and utility of the measures, the settings and scope/impact on contributions, and the usefulness of the new measure for both deletions and value updates, as discussed in the previous items. 
}
\end{authorreply}

\textbf{Required changes for revision:}
\begin{reviewcomment}
O1, O2, O3, O4.
 \end{reviewcomment}
\begin{authorreply}
\rrevtwo{
All have been addressed, as discussed above. We thank the reviewer for the comments
  and highly appreciate  that the resulting revision is a considerable
  improvement over the original submission.
}
\end{authorreply}

\section*{Reviewer 3}

\begin{reviewcomment}
O1: Some parts of the paper should better scope what is covered by the proposal. This is a measure of inconsistency wrt to a set of given rules. Many errors can easily be missed by the given constraints. The title and the abstract are much more general and should be made more clear.
 \end{reviewcomment}
\begin{authorreply}
\rrevthree{Indeed, we adopt the meaning of ``inconsistency'' in the
    context of integrity constraints. As far as we know, identifying
    inconsistency with constraint violation is a conventional
    technical term
    (e.g.,~\cite{DBLP:series/synthesis/2011Bertossi}). Of course, one
    could also interpret inconsistency in a broader sense, as the
    reviewer suggests. We have added clarifications in the {\bf
     Abstract} and {\bf Section~\ref{sec:introduction}}, but left the
    title unchanged for brevity.  }
%\ester{We did not address this comment, but we can say that \textbf{inconsistency} is usually defined via violation of constraints.}

%\sudeepa{updated abstract/intro}\red{CHECK}
\end{authorreply}

\begin{reviewcomment}
O2: While rules have been largely studied in data repairing, there is evidence that rule based detection plays a minor role in the error detection process, see for example
Abedjan et al - Detecting Data Errors: Where are we and what needs to be done? Proc. VLDB Endow. 9(12): 993-1004 (2016)
The proposal would be much stronger if authors could extend it beyond rule based measures
 \end{reviewcomment}
\begin{authorreply}
%\red{COPIED FROM RESPONSE LETTER}
  \rrevthree{ As we said in the rebuttal, we are aware of this work but missed to cite this in our original submission. We thank the reviewer for pointing out this work -- we
    now cite it in the
    revised version. Indeed,
    inconsistency measures (as we define them) quantify the extent to which constraints
    are violated. Hence, there are challenges in data cleaning and
    data quality management that are beyond the scope of this work (\textbf{Please see "other related work" in Section~\ref{sec:introduction}}).

    That said, one can use an inconsistency measure in any cleaning
    system, adopting any correction mechanism whatsoever, for
    providing a specific view of the progress: the status of (soft)
    constraint satisfaction (rather than the status of general
    truthfulness). To illustrate this point, we have a added a new
    case study with the HoloClean
    system~\cite{DBLP:journals/pvldb/RekatsinasCIR17}, where we
    provided it with increasingly larger sets of constraints and
    applied the measures after each cleaning
    application. Interestingly, the measures that have a good
    theoretical behavior are also well capturing progress in the HoloClean case study.
    HoloClean
    uses soft rules and a statistical approach for automatic data
    cleaning.  Please see
    \textbf{Section~\ref{sec:exp:holoclean}} and also the new remarks in the \textbf{Introduction (Section~\ref{sec:introduction})}.}

\sudeepa{\red{@Ihab}: please check this.}

\end{authorreply}

\begin{reviewcomment}
O3: Even if we focus only on rules, the hard problem is to have a measure for the cleaning systems/algorithms that are based on tuple updates, such as [13,18,31]. However, the main result here is on tuple deletion only. The arguments in section 6.2 are sound and justify the proposal, but they are known in database repair literature. Given that the properties are reasonable (S1), it is not clear what is the solution to the problem, but the paper leaves the feeling that only the problem has been solved here, but for a setting that it's not the one that we see in (rule based) applications.
 \end{reviewcomment}
\begin{authorreply}
  \rrevthree{ Thank you for this comment. 
  %We apologize upfront for  repeating some of the statements from the rebuttal. As we said there, we believe that the work and paper are valuable 
  We have significantly elaborated on this concern in several places of the paper (including \textbf{Sections~\ref{sec:introduction}, \ref{sec:rational} (Remark at the end), and \ref{sec:experiments}}). Please also see our responses regarding potential impact of our contributions in response to Metareviewer-Comment1, and to \textbf{Reviewer1-author feedback} or \textbf{Reviewer2-O2}.}
  
  \rrevthree{ In particular,
  the concept and framework of inconsistency measures go beyond tuple deletion, and
    particularly to attribute updates, for the following reasons.
    \begin{itemize}
    \item The general properties are orthogonal to the repair
      operations.
    \item The specific measures that we present and analyze (as well
      as future measures) can be used for quantifying inconsistency no
      matter what operations are allowed.  
      %As we said in the rebuttal,
      Any repair system, supporting any type of repairing operations
      whatsoever, could adopt measures such as $\Imr$ (corresponding
      to the maximal consistent subset) and $\Ilmr$ (the linear
      relaxation). It is just that some theoretical results only hold for tuple deletion, e.g., continuity and progression are
      provably guaranteed only for deletion operations.
    \item Indeed, the experimental study
      (Section~\ref{sec:experiments}) shows that the measures that
      well behave theoretically also exhibit a good empirical
      behavior going beyond tuple deletions, 
      %even though 
      as our error models capture attribute updates.
      %rather than tuple insertions (to be remedied by tuple deletions). 
      Moreover, our case study with HoloClean shows the
      value of our contribution in a system that automatically updates
      attribute values.
    \item In Section~\ref{sec:more-general} we discuss guarantees for
      attribute updates. We explain there that there is a measure that
      satisfies all of the properties---this is correspondent of
      $\Imr$ (minimum update repair). Yet, this measure might be  hard
      to compute, and finding a tractable relaxation (such as $\Ilmr$)
      remains an open problem.
      \end{itemize}}
\end{authorreply}

\textbf{Additional remarks:} 
\begin{reviewcomment}
A1. why in example 1 "an automated data cleaning alg cannot detect these changes"?
 \end{reviewcomment}
\begin{authorreply}
\rrevthree{
We have rephrased this sentence. To clarify: when the clean database is not available, if only two versions of noisy databases are given, it is non-trivial to detect which one is `more noisy' or if we are making progress in cleaning by a repair system in going from one to the other, which an inconsistency measure helps us to decide. 
}

\sudeepa{check}
%\sudeepa{Add the meaning nevertheless.}
\end{authorreply}

\begin{reviewcomment}
A2. 
typo `probabable` in sec 1
 \end{reviewcomment}
\begin{authorreply}
\rrevthree{
Fixed.
}
\end{authorreply}



\textbf{Response to author feedback:}
\begin{reviewcomment}
The feedback confirms my understanding of the paper and clarifies some aspects. I think the authors have an opportunity to show that their work as a bigger scope in the revision step.
 \end{reviewcomment}
\begin{authorreply}
  \rrevthree{ We are very grateful for this opportunity.  We believe
    that the paper, and more importantly the research it reports, have
    considerably improved in this revision due to the valuable reviews.}
\end{authorreply}

\textbf{Required changes for a revision}
\begin{reviewcomment}
Based on your answers to O2 and O3, I think you can definitely improve the discussion of such aspect. However, the paper would be stronger if you could also provide experiments that go beyond error detection and strict rules (to better address O2) and that show the limits of the solution with update repairs with any of the available data repair system and one of the scenarios from the literature (to better address O3).
 \end{reviewcomment}
\begin{authorreply}
  \rrevthree{  Indeed, the experimental study underwent a considerable
    extension and improvement, including experiments with value updates. Please see our answers to Reviewer3-O2 and Reviewer3-O3. 
  }
\end{authorreply}

\cut{
=======================
\begin{reviewcomment}
  (Typos and minor errors.)
 \end{reviewcomment}
\begin{authorreply}
  We have fixed all minor errors pointed out by the reviewer, and we
  applied all additional suggestions. Thank you.
\end{authorreply}
}
%\setcounter{footnote}{0}
%\end{document}

==> response_saved.tex <==

%\documentclass[10pt,a4paper,twoside]{article}
\usepackage[dvipsnames]{xcolor}
%\usepackage{geometry}
%\usepackage{hyperref}
\usepackage{cite}
\geometry{margin=1.2in}

\newcommand{\rev one}[1]{{\color{violet}#1}}
\newcommand{\revtwo}[1]{{\color{red}#1}}
\newcommand{\revthree}[1]{{\color{blue}#1}}


%\newcommand{\eat}[1]{}

%\setlength{\parindent}{0em}
%\setlength{\parskip}{1em}

\newcommand{\depset}{\mathrm{\Delta}}
\newcommand{\sch}[1]{\mathbf{#1}}
\newcommand{\scs}{\sch{S}}

\newcommand{\mathsc}[1]{{\normalfont\textsc{#1}}}
\def\fdparam#1#2{\langle #1,#2\rangle}
\def\sharpsrep{\mathsc{\#SRep}}
\def\sharpsrepfd#1#2{\mathsc{\#SRep}\fdparam{#1}{#2}}

\newenvironment{reviewcomment}
{\vskip 0.2em\par\noindent\textbf{Comment:}\it}{\par}

\newenvironment{authorreply}
{\vskip 0.5em\par\noindent\textbf{Reply:} \color{purple}}
{\vskip 1em}





\cut{

%\documentclass[10pt,a4paper,twoside]{article}
\usepackage[dvipsnames]{xcolor}
\usepackage{geometry}
\usepackage{hyperref}
\usepackage{cite}
\geometry{margin=1.2in}

\newcommand{\revone}[1]{{\color{violet}#1}}
\newcommand{\revtwo}[1]{{\color{red}#1}}
\newcommand{\revthree}[1]{{\color{blue}#1}}

\newcommand{\eat}[1]{}

%\setlength{\parindent}{0em}
%\setlength{\parskip}{1em}

\newcommand{\depset}{\mathrm{\Delta}}
\newcommand{\sch}[1]{\mathbf{#1}}
\newcommand{\scs}{\sch{S}}

\newcommand{\mathsc}[1]{{\normalfont\textsc{#1}}}
\def\fdparam#1#2{\langle #1,#2\rangle}
\def\sharpsrep{\mathsc{\#SRep}}
\def\sharpsrepfd#1#2{\mathsc{\#SRep}\fdparam{#1}{#2}}

\newenvironment{reviewcomment}
{\vskip 0.2em\par\noindent\textbf{Comment:}\it}{\par}

\newenvironment{authorreply}
{\vskip 0.5em\par\noindent\textbf{Reply:} \color{purple}}
{\vskip 1em}
}


\def\e#1{\emph{#1}}

%\begin{document}

%\thispagestyle{empty}

\newcommand{\letterpartitle}[1]{\vskip1em\noindent {\bf #1.\,}}

\begin{center}
{\large \textbf{Properties of Inconsistency Measures for Databases}}\vskip1em
\def\thefootnote{\fnsymbol{footnote}}

\def\au#1{\textbf{#1}} Anonymous Author(s)


\vskip3em



{\underline{\large Cover Letter for Revision}}\vskip3.5em
\end{center}

\setcounter{footnote}{0}

%\noindent Dear JCSS editor and referees,\\

